How Does the Task Landscape Affect MAML Performance?

Model-Agnostic Meta-Learning (MAML) has become increasingly popular for training models that can quickly adapt to new tasks via one or few stochastic gradient descent steps. However, the MAML objective is significantly more difficult to optimize compared to standard non-adaptive learning (NAL), and little is understood about how much MAML improves over NAL in terms of the fast adaptability of their solutions in various scenarios. We analytically address this issue in a linear regression setting consisting of a mixture of easy and hard tasks, where hardness is related to the rate that gradient descent converges on the task. Specifically, we prove that in order for MAML to achieve substantial gain over NAL, (i) there must be some discrepancy in hardness among the tasks, and (ii) the optimal solutions of the hard tasks must be closely packed with the center far from the center of the easy tasks optimal solutions. We also give numerical and analytical results suggesting that these insights apply to two-layer neural networks. Finally, we provide few-shot image classification experiments that support our insights for when MAML should be used and emphasize the importance of training MAML on hard tasks in practice.

==> NeurIPS/Discussion.tex <==
\section{Discussion}
% \textbf{Discussion -- Why MAML.} 
Our work highlights the importance of hard tasks to the success of MAML. We show that MAML outperforms standard training (NAL) in both linear and nonlinear settings by finding a solution that outperforms NAL on the more-difficult-to-optimize (hard) tasks, as long as they are sufficiently similar. 
Our results provide theoretical justification for the empirical benefits of focusing on the hard tasks while training meta-learning methods \citep{zhou2020expert,sun2020meta} and give intuition to practitioners on when they can save computational resources by using standard NAL for meta-learning instead of the more expensive MAML. Still, the notions of task hardness and similarity we use in our experiments cannot be applied to all multi-task learning problems. We leave the further development of methods to measure task hardness and similarity to future work.

% , noting that some works have made initial strides on this problem in the context of deep learning \citep{gagne2019principled, tran2019transferability, venkitaraman2020task}.

% Our work further recognizes the importance of the similarity of the hard tasks -- if the hard tasks in an environment are very dissimilar, then MAML barely gains over NAL.

% \textbf{Limitations.}
% % Our notions of task hardness and similarity here are environment-specific.
% The notions of task hardness and similarity we use in our experiments cannot be applied to all multi-task learning problems. We leave the development of more universal methods to measure task hardness and similarity in deep learning to future work \citep{gagne2019principled, tran2019transferability, venkitaraman2020task}. 
% We also leave it up to practitioners to decide how they want to use our insights to determine when to use MAML, depending on their unique computational constraints and performance goals.

% which may involve 
% . Making this determination naturally involves biases, which may result in poor model performance on hard tasks if NAL is incorrectly chosen. 
% We leave robust methods for gauging the task landscape for future work.



%TODO for ICLR:

% insert new simulation
% be clear on definition of task hardness
% how to make results seem less incremental?

==> NeurIPS/Experiments.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Experiments} \label{section:experiments}
\vspace{-2mm}
% We aim to empirically answer three questions: 1) In settings with similar hard tasks, does MAML outperform NAL on the hard tasks? 2)
We next experimentally study whether our observations generalize to problems closer to those seen in practice. 
We consider image classification on the Omniglot \citep{lake2019omniglot} and FS-CIFAR100 \citep{oreshkin2018tadam} datasets. Following convention, tasks are $N$-way, $K$-shot classification problems, i.e., classification problems among $N$ classes where $K$ labeled images from each class are available for adapting the model.
% In all of our experiments, $N\!=\!5$ and $K \in \{1,10\}$.
For both the Omniglot and FS-CIFAR100 experiments, we use the five-layer CNN used in \cite{finn2017model, vinyals2016matching}. NAL is trained equivalently to MAML with no inner loop and $n\!=\!n_1\!+\!n_2$. 
%We sample two task instances on each round, and train for 10,000 outer loop iterations. 
Further details and error bounds are in Appendix \ref{app:experiments}.
% number of samples/maml s samples for NAL, fine-tuning




\textbf{Omniglot.}
Omniglot contains images of 1623 handwritten characters from 50 different alphabets. Characters from the same alphabet typically share similar features, so are harder to distinguish compared to characters from differing alphabets.
% images  a class is a set of handwritten images of the same character.
% so at a high level our goal is to distinguish characters. 
% There are 1623 characters from 50 different alphabets in the dataset. %, and %including ancient, modern, and fictional alphabets. 
% characters within each alphabet generally share similar structure, while this structure varies substantially across alphabets. %Since the hardness of a classification task depends on the distinguishability of the classes \citep{36578}, 
% These semantic relationships among the Omniglot characters thus provide a natural means to construct easy and hard tasks \citep{zhou2020expert}. 
We thus define easy tasks as classification problems among characters from {\em distinct} alphabets, and hard tasks as classification problems among characters from the {\em same} alphabet, consistent with prior definitions of {\em semantic hardness} \citep{zhou2020expert}. Here we use $N\!=\!5$ and $K\!=\!1$.
%, thus $n_2 \!=\! m\! =\! 5$. 
For NAL, we include results for $K=10$ (NAL-10) in addition to $K=1$ (NAL-1). 
We split the 50 alphabets into four disjoint sets: easy train (25 alphabets), easy test (15), hard train (5), and hard test (5). During training, tasks are drawn by first choosing `easy' or `hard' with equal probability. If `easy' is chosen, 5 characters from 5 distinct alphabets among the easy train alphabets are selected. If `hard' is chosen, a hard alphabet is selected from the hard train alphabets, then $N\!=\!5$ characters are drawn from that alphabet. After training, we evaluate the models on new tasks drawn analogously from the test (unseen) alphabets as well as the train alphabets. 
% \begin{table}[t]
% \caption{Omniglot accuracies} \label{table:1}
%  \vspace{-2mm}
% \begin{center}
% \begin{tabular}{llllll}
%   & & \multicolumn{2}{c}{{Train Tasks}}  &  \multicolumn{2}{c}{{Test Tasks}}               \\
% \cmidrule(r){3-4}
%     \cmidrule(r){5-6}
% $r_H$ &{Alg}  &{Easy} &{Hard} &{Easy} &{Hard}\\
% \hline 
% Small &MAML         & $99.2 \pm .5$ & $99.1 \pm .1$ & $98.1 \pm .1$ & $95.4 \pm .3$ \\
% Small &NAL-1             &$69.2$  & $46.0$ & $55.8$ & $45.8$ \\
% Large & NAL-10            & $70.0$ & $45.3$ & $67.2$ & $47.9$ \\
% \hline 
% Large &MAML         & $99.2 \pm .1$ & $96.0 \pm .6$ & $98.0 \pm .1$ & $81.2 \pm .3$ \\
% Large &NAL-1             & $69.4$ & $41.5$ & $57.8$ & $45.2$ \\
% Small &NAL-10             &$70.2$  & $44.0$ & $67.8$ & $48.9$ \\
% \end{tabular}
% \end{center}
% \vspace{-4mm}
% \end{table}


\begin{table}[t]
\begin{minipage}{.5\linewidth}
% \subfloat[Omniglot accuracies with  95\% confidence intervals.]{
 \caption{Omniglot accuracies.} % with  95\% confidence intervals
 \vspace{-4mm}
 \label{table:1}
%  \vspace{-3mm}
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{llllll}
\toprule
   \multicolumn{2}{c}{{Setting}} & \multicolumn{2}{c}{{Train Tasks}}  &  \multicolumn{2}{c}{{Test Tasks}}          \\
\cmidrule(r){1-2}
\cmidrule(r){3-4}
    \cmidrule(r){5-6}  
$r_H$ &{Alg.}  &{Easy} &{Hard} &{Easy} &{Hard} \\
\hline 
Large &MAML         & $99.2$ & $96.0$ & $98.0$ & $81.2$  \\
Large &NAL-1             & $69.4$ & $41.5$ & $57.8 $ & $45.2$  \\
Large & NAL-10            & $70.0$ & $45.3$ & $67.2$ & $47.9$ \\
\hline 
Small &MAML         & $99.2$ & $99.1$ & $98.1$ & $95.4$ \\
Small &NAL-1             &$69.2$  & $46.0$ & $55.8$ & $45.8$ \\
Small &NAL-10             &$70.2$  & $44.0$ & $67.8$ & $48.9$  \\
\bottomrule
\end{tabular}
% \begin{tabular}{llllll}
%   & & \multicolumn{2}{c}{{Train Tasks}}  &  \multicolumn{2}{c}{{Test Tasks}}               \\
% \cmidrule(r){3-4}
%     \cmidrule(r){5-6}
% $r_H$ &{Alg}  &{Easy} &{Hard} &{Easy} &{Hard}\\
% \hline 
% Large & MAML & $99.2$ & $96.0$ & $98.0$ & $81.2$ \\
% Large & NAL-1             & $49.1$ & $31.4$ & $48.2$ & $31.1$ \\
% Large & NAL-10            & $70.0$ & $45.3$ & $67.2$ & $47.9$ \\
% \hline 
% Small &MAML         & $99.2$ & $99.1$ & $98.1$ & $95.4$ \\
% Small &NAL-1           &$48.7$  & 30.1 & $48.3$ & 29.4 \\
% Small &NAL-10             &$70.2$  & 44.0 & $67.8$ & 48.9 \\
% \end{tabular}
% \end{sc}
\end{small}
\end{center}
\end{minipage}
% \vspace{-5mm}
% \vspace{-1mm}
% \end{table}
% \subfloat[FS-CIFAR100 test accuracies with 95\% confidence intervals.]{
% \begin{table}[t]
\begin{minipage}{0.5\linewidth}
 \caption{FS-CIFAR100 accuracies.} % with 95\% confidence intervals
 \vspace{-4mm}
 \label{table:fs-cifar}
%  \vspace{-3mm}
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{llllll}
\toprule
   \multicolumn{2}{c}{{Setting}} & \multicolumn{2}{c}{{Train Tasks}}  &  \multicolumn{2}{c}{{Test Tasks}}          \\
\cmidrule(r){1-2}
\cmidrule(r){3-4}
    \cmidrule(r){5-6}  
$p$ &{Alg.}  &{Easy} &{Hard} &{Easy} &{Hard} \\
\hline
    \multirow{2}{*}{0.99} & NAL     &  78.2 & 9.9  &  74.8  & 9.5  \\
    & MAML     & 92.9 & 50.1 & 84.6     & 21.7   \\ %90.1 & 55.2 & 85.3     & 21.7  
    \hline
    \multirow{2}{*}{0.5} & NAL & 81.9   & 9.5 & 76.5 &  8.6    \\
    & MAML     & 93.6 & 41.1 & 84.3 & 17.9   \\ %94.7 & 48.5  & 85.3 & 21.6 
    \hline
    \multirow{2}{*}{0.01} & NAL &  82.4 & 7.6 &   76.9  & 8.2  \\
    & MAML     & 94.0 & 15.7  &   85.0   & 11.8    \\ %8.9 &   79.5   & 6.6 
    \bottomrule
\end{tabular}
\end{small}
\end{center}
\end{minipage}
\end{table}


% \subfloat[FS-CIFAR100 test accuracies with 95\% confidence intervals.]{
% %   \caption{\begin{small}FS-CIFAR100 test accuracies with 95\% confidence intervals.
% %   \end{small}}
%   \label{table:fs-cifar}
%  \centering
%   \begin{small}
  
%   \begin{tabular}{cccccc}
%     \toprule
%     % \multicolumn{2}{c}{Part}                   \\
%     % \cmidrule(r){1-2}
%     $p$ & Algorithm    & Easy-Train  &  Hard-Train  & Easy-Test  &  Hard-Test & Runtime (s) \\
%     \midrule
%     \multirow{2}{*}{0.5} & NAL & 83.5   & 8.5 & 78.7 &  7.3    \\
%     & MAML     & 94.7 & 48.5  & 85.3 & 21.6    \\
%     \midrule
%     \multirow{2}{*}{0.99} & NAL &  84.0 & 5.8 &   78.5  & 9.5  &  \\
%     & MAML     & 95.2 & 8.9 &   79.5   & 6.6    \\
%     \midrule
%     \multirow{2}{*}{0.01} & NAL     &  80.11 & 9.2  &  78.5  & 8.0  \\
%     & MAML     & 90.1 & 55.2 & 85.3     & 21.7   \\
%     \bottomrule
%   \end{tabular}
%   \end{small}
%   }
% \end{table}
% [0.85321647 0.21638721]



%and \ref{table:2}.
% In particular, for each classification problem, there are 5 classes (characters) from the same or different alphabets, depending on the task's hardness. 

%Both NAL and MAML train for 25,000 iterations with a batch size of 4. 

Table \ref{table:1} gives the average errors  after completing training for two experiments: the first (Large) when the algorithms use all 5 hard train and test alphabets, and the second (Small) when the algorithms use only one hard train alphabet (Sanskrit) and one hard test (Bengali). The terms `Large' and `Small' describe the hypothesized size of $r_H$ in each experiment: the optimal solutions of hard tasks drawn from ten (train and test) different alphabets are presumably more dispersed than hard tasks drawn from only two (train and test) similar alphabets. By our previous analysis, we expect MAML to achieve more gain over NAL in the Small $r_H$ setting. Table \ref{table:1} supports this intuition, as MAML's performance improves significantly with more closely-packed hard tasks (Small), while NAL's does not change substantially. Hence, {\em MAML's relative gain over NAL increases with smaller $r_H$}.

% \subsection{Additional Experimental Details}

% We use the same 4-layer convolutional neural network architecture as in \citep{finn2017model}, using code adapted from the repository available at \url{https://github.com/AntreasAntoniou/HowToTrainYourMAMLPytorch} that implements in Pytorch \url{https://pytorch.org/} the experiments in the paper \cite{antoniou2018train}. We ran SGD on the MAML and NAL objectives using 10 target samples per class for MAML, i.e. $n_1 = 5 \times 10$. Likewise,  $n= n_1 + 5\times n_2$ samples were used in each task to update $\mathbf{w}_{NAL}$ on each iteration, for $n_2 = 5\times K$. Eight tasks were drawn on each iteration for a total of 20,000 iterations. Meta-learning rates were tuned to be $10^{-6}$ for NAL and $10^{-3}$ for MAML. To select the alphabets corresponding to hard tasks, we ran MAML on tasks drawn from all 50 Omniglot alphabets, and took the 10 alphabets with the lowest accuracies. The train/test splits were then random among the remaining alphabets.

% \textbf{Conclusion.} We have analyzed the performance of MAML and NAL for linear regression with a $d$-dimensional regressor and a two-layer linear neural network. Our main insight is that the hard tasks must be closely packed and far from the the easy tasks in order for MAML to improve non-trivially over NAL. We have provided experimental results to support these conclusions, including for nonlinear networks.

% Before executing this experiment, we ran MAML on `hard' classification problems drawn from each of the 50 alphabets, and designated the 10 alphabets with the worst accuracy to constitute the hard tasks. The other 40 alphabets were used to sample easy tasks. 
% Specifically, we used 30 of the easy alphabets to sample easy tasks during training, and one or five of the hard alphabets to sample hard tasks. The test tasks are classification problems drawn from the remaining alphabets.

% In Table $\ref{}$, we
% To choose the alphabets for the hard tasks, we

% We first run MAML on
% To avoid overfitting, 

% need NAL to stay the same between 1 and 5, maml should get worse

%and significantly more difficult to distinguish, as others have noticed \cite{48798}. This allows for a natural construction of tasks with varied `semantic hardness' as defined in \cite{zhou2020expert}, which establishes that easy tasks are classification problems among classes 

% Based on this definition of hardness, we define easy tasks as $N$-way classification problems among characters from distinct alphabets, and hard tasks as $N$-way classification problems among characters from the same alphabet.


% - Measure distance traveled during update for hard task vs easy tasks

% - Measure distance traveled during update for hard tasks when the hard tasks are diverse vs when they are not

% - introduce regularizer that punishes variance among the hard task local solutions? but how to determine hard tasks? weight regularizer by loss? first try it when we know what the hard tasks are

% - 

%1) In a linear regression setting with easy and hard tasks, how does task hardness, indicated by the variance of the tasks' data, impact performance for NAL and MAML? 2) In a similar setting, how do the locations of the tasks' optimal solutions affect performance? 3) Do these patterns generalize beyond linear regression to more complex settings?



% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Task  & Hard Task  \\ \hline
% MAML      & 0.98 & 0.97 \\ \hline
% NAL       &  0.73  & 0.51  \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - standard CNN}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Task  & Hard Task  \\ \hline
% MAML      & 0.83 & 0.57 \\ \hline
% NAL       &  0.60  & 0.38  \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - reduced CNN}
% \end{table}
% Note that NAL has 15 shots, MAML has 1 shot
% When adding more tasks of each type, accuracies are within 5 points of the single-task accuracy for that type.

% MAML gets to (98,95) when using all the alphabets for training, and (96,85) for test classes. NAL still at (71,44) training, (78,42) testing in this case

% When there is only one hard task, MAML performs just as well on the hard task as it does on the easy tasks:
% \begin{table}[h]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Tasks (Avg)  & Hard Task  \\ \hline
% MAML      & 98.5 & 98.3 \\ \hline
% NAL       &  74.0  & 51.0  \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - full CNN}
% \end{table}

% But when there are 10 hard tasks (which presumably are dispersed), MAML struggles on them on average, while NAL does not change much (Table 4):
% \begin{table}[h]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Tasks (Avg)  & Hard Tasks (Avg)  \\ \hline
% MAML   &  98.7 & 93.3   \\ \hline
% NAL    &  71.9 & 50.2      \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - full CNN}
% \end{table}

% Meanwhile, when we decrease the dispersion of the easy tasks, there is no significant change
% \begin{table}[h]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Tasks (Avg)  & Hard Tasks (Avg)  \\ \hline
% % MAML    98.15  & 90.0 &  \\ \hline
% % NAL     73.7  &  50.5  &   \\ \hline
% MAML    99.2 & 93.0 &  \\ \hline
% NAL     71.0  &  50.2  &   \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - full CNN}
% \end{table}

% Counterargument 1: as you increase the number of iterations, MAML eventually learns even the 10 hard tasks very well (75,000 iterations, at least 95\% accuracy). But we can still see relative performance differences

% Counterargument 2: We are training and testing on essentially the same data, obviously MAML learns the one hard task better because one task is easier to overfit to than 10 tasks

% Counterargument 3: These results are for m=15 for NAL, m=1 for MAML, which makes it much easier for NAL. NAL does terribly with m=1.

% \subsection{Beyond Linear Regression}


% to do: TODO: 
% run real experiments, 2 dimensions, accounting for convergence, include new testing tasks
% - test case where hard and easy tasks have the same center, use same dispersion of both types of tasks. shows what khodak said.
% - test case where hard and easy tasks have the same center, use different dispersion of the hard tasks, keep easy tasks spread out. shows that hard tasks being close is not enough for maml improvement over erm - must have dif center too.
% - test case where easy and hard tasks have different center, use different dispersion of the hard tasks, with easy tasks spread out
% - test case where easy and hard tasks have different center, use different dispersion of the easy tasks, with hard tasks spread out


% \begin{enumerate}
%     \item $U_H = U_E$, both vary together.
%         \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{20tasks_bothVary.png}}
% \caption{Theoretical results for setting described above, for values of $U_H = U_E \in \{-9,-8, ..., 10\}$.  In this case the hard tasks and easy tasks are close together depending on the value of $U_H = U_E$. All results are averages over 10 trials. For the random initialization, here $D=10$. \textbf{As we can see from the middle plot, having all of the tasks close together results in substantial improvement for MAML over the random initialization, as claimed by Khodak et al. 2019 and others. However, this condition does not give improvement for MAML over standard supervised learning (NAL), which the prior works do not point out.}}
% \label{20tasks_both}
% \end{center}
% \vskip -0.2in
% \end{figure}
    
%     \item $U_H = 10$, $U_E$ varies. 
%         \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{20tasks_easyVaries.png}}
% \caption{Theoretical results for setting described above, for values of $U_E \in \{-9,-8, ..., 10\}$ and $U_H$ fixed at 10. In this case the hard tasks are always dispersed, while the easy tasks are close together depending on the value of $U_E$. All results are averages over 10 trials. As we can see, when the easy tasks are close together, MAML slightly outperforms NAL, but not by much, and the improvement over the random initialization is not as significant as in other cases, for both NAL and MAML. \textbf{Thus, having only the easy tasks close together is not particularly helpful for MAML.}}
% \label{20tasks_easy}
% \end{center}
% \vskip -0.2in
% \end{figure}
    
%     \item $U_H$ varies, $U_E = 10$. 
%     \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{20tasks_hardVaries.png}}
% \caption{Theoretical results for setting described above, for values of $U_H \in \{-9,-8, ..., 10\}$ and $U_E$ fixed at 10. In this case the easy tasks are always dispersed, while the hard tasks are close together depending on the value of $U_H$. All results are averages over 10 trials. As we can see, when the hard tasks are close together, MAML drastically outperforms NAL and the random initialization, because it initializes close to the hard tasks, thus performs well on those, and also performs well on the easy tasks, since they can be reached by one step of gradient even if they are far away. \textbf{Thus, having the hard tasks close together is the key to MAML's success. If the easy tasks are also close together, then NAL also performs well (as seen in Figure \ref{20tasks_both}), but it fails when the easy tasks are dispersed, unlike MAML, which is robust to the location of the easy tasks.}}
% \label{20tasks_hard}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \item $U_H$ varies, $U_E = 10$, hard tasks and easy tasks have the same center. 
%     \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{20tasks_hardVaries_centered.png}}
% \caption{Theoretical results for setting described above, except that for the hard tasks, $w_{i}^\ast \sim \mathcal{U}(-U_H, U_H)$, for $U_H \in \{0.5,1,1.5,...,9.5\}$, and $U_E$ fixed at 10. In this case the easy tasks are always dispersed, while the hard tasks are close together depending on the value of $U_H$. All results are averages over 10 trials. As we can see, although the hard tasks are close together while the easy tasks are dispersed, \textbf{MAML and standard supervised learning perform similarly because the hard tasks and the easy tasks have the same center.}}
% \label{20tasks_hard}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \item $U_H$ varies, $U_E$ fixed, hard tasks and easy tasks have a different center. 
%     \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{20tasks_hardVaries_uncentered.png}}
% \caption{Theoretical results for setting described above, except that for the hard tasks, $w_{i}^\ast \sim \mathcal{U}([-10,-10+U_H] \cup [-U_H,0])$, for $U_H \in \{0.25,0.5,0.75,...,5\}$, and the easy tasks are drawn as $w_{i}^\ast \sim \mathcal{U}([0,10])$. In this case the hard tasks are dispersed but have center (-5) very different from the center of the easy tasks (5). \textbf{The difference in the centers of the tasks gives MAML an advantage over standard supervised learning, but it is not very significant because the hard tasks are dispersed.}}
% \label{20tasks_hard}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \end{enumerate}

% In summary, the two necessary and sufficient conditions for MAML to confer an advantage over NAL are that the hard tasks have optimal solutions that are (1) close together and (2) far from the center (average) of the optimal solutions of the easy tasks, assuming appropriate choice of inner loop step size $\alpha$ and sufficient disparity between $\rho_H$ and $\rho_E$. We provide experiments, as well as theoretical analysis, for small $m$ in the Appendix.

% easy tasks are 

% MAML, training accs (easy, hard): [0.96771157 0.3701961]

% NAL, training accs (easy, hard):
% [0.9598738  0.32611108]

% todo: accs should be the same for erm hard and easy tasks.

% We need to e



% \begin{table}[h]
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{} & Easy Tasks (Avg)  & Hard Tasks (Avg)  \\ \hline
% % MAML    98.15  & 90.0 &  \\ \hline
% % NAL     73.7  &  50.5  &   \\ \hline
% MAML    99.2 & 93.0 &  \\ \hline
% NAL     71.0  &  50.2  &   \\ \hline
% \end{tabular}
% \caption{Omniglot test accuracies - full CNN}
% \end{table}


% \begin{table}
%   \caption{\begin{small}FS-CIFAR100 test accuracies with 95\% confidence intervals.
%   \end{small}}
%   \label{table:fs-cifar}
%  \centering
%   \begin{small}
  
%   \begin{tabular}{ccccccc}
%     \toprule
%     % \multicolumn{2}{c}{Part}                   \\
%     % \cmidrule(r){1-2}
%     $p$ & Algorithm    & Easy-Train  &  Hard-Train  & Easy-Test  &  Hard-Test & Runtime (s) \\
%     \midrule
%     \multirow{2}{*}{0.5} & NAL & 83.5   & 8.5 & 78.7 &  7.3  &  \\
%     & MAML     & 94.7 & 48.5  & 85.3 & 21.6  &  \\
%     \midrule
%     \multirow{2}{*}{0.99} & NAL &  84.0 & 5.8 &   78.5  & 9.5  &  \\
%     & MAML     & 95.2 & 8.9 &   79.5   & 6.6  &  \\
%     \midrule
%     \multirow{2}{*}{0.01} & NAL     &  80.11 & 9.2  &  78.5  & 8.0 &  \\
%     & MAML     & 90.1 & 55.2 & 85.3     & 21.7  & \\
%     \bottomrule
%   \end{tabular}
%   \end{small}
% \end{table}

\textbf{FS-CIFAR100.} FS-CIFAR100 has 100 total classes that are split into 80 training classes and 20 testing classes. We further split the 600 images in each of the training classes into 450 training images and 150 testing images in order to measure test accuracy on the training classes in Table \ref{table:fs-cifar}. Here we use $N$ and $K$ as proxies for hardness, with larger $N$ and smaller $K$ being more hard as the agent must distinguish more classes with fewer training samples/class. Specifically, easy tasks have $(N,K) = (2,10)$, and the hard tasks have $(N,K) = (20,1)$.
During training, hard tasks are sampled with probability$~p$ and easy tasks with probability $1\!-\!p$. Observe that the largest performance gains for MAML in Table \ref{table:fs-cifar} are on the hard tasks, consistent with our conclusion that MAML outperforms NAL primarily by achieving relatively high accuracy on the hard tasks.
However, the improvement by MAML on the hard tasks disappears when the hard tasks are scarce $(p=0.01)$, supporting the idea of oversampling hard tasks during training in order to improve MAML performance \citep{zhou2020expert,sun2020meta}.


% If easy, sample 2 classes from among the training classes, and shuffle their labels. Select images from each class. If hard, sample 20 classes from among the training classes, and shuffle their labels. During testing: Sample training tasks: For easy tasks, sample 2 classes among the training classes,  shuffle their labels, sample 10 samples/class, take 1 gradient step, evaluate the loss after update. For hard tasks, do the same but sample 20 classes, shuffle the labels and sample 1 image/class.
% For the test tasks, do the same among the test classes.

%   Issues: If we shuffle the labels, then NAL has no hope. But if we don't shuffle the labels, then there is no need to learn how to adapt (because we can find a model that performs well on the dataset without adaptation) so you would not consider using meta-learning in this setting to begin with...

% best so far: 73%, lr = 0.01, 5 steps, 1 shot. 5 shots gets to 79%. need to try with different lr.



% \textbf{Possible algorithms (prescriptive):}
%  \begin{itemize}
% \item Run MAML. On the each inner loop, take an SGD step using some minibatch as usual. If the loss on the target set after this adaptation of the model is small enough AND the model changed significantly enough during the update, then throw away this task (since these factors suggest it is easy). Instead of throwing it away completely, we could compute a first-order gradient for this task as opposed to second order (but only marginal efficiency gains, often we don't use second-order anyway, and requires more parameter tuning). 
% \item You start by running NAL. If the gradients are sufficiently contradictory to each other, you switch to MAML... doesn't make sense because tasks could be all easy and heterogeneous.
% \item Reptile-like method: instead of MAML, interpolate between the estimated solutions of the hard tasks after inner loop update... weight interpolation coefficient by the loss.
% \item Add a regularizer that encourages 
%  \end{itemize}


==> NeurIPS/Geography.tex <==

% and that each $\mathbf{\Sigma}_i$ is diagonal.

% {\em (i) (Intuition on Hardness)} 
% % We first clarify our notion of task hardness. 
% Recall that task hardness depends on how quickly gradient descent can traverse the loss function of the task, with harder tasks requiring more steps of gradient descent to reach an optimal solution. {\em Since the loss functions $f_i$ are convex, the speed with which gradient descent traverses each $f_i$ depends on 
% % the steepness of $f_i$, which in turn is determined by 
% the minimum eigenvalue of the Hessian of $f_i$ (in this setting, $\mathbf{\Sigma}_i$).}

%
% The Hessian of $f_i$ is $\mathbf{\Sigma}_i$, so $\mathbf{\Sigma}_i$ determines the steepness of $f_i$ and therefore the hardness of task $i$. 
%
% Thus, the hardness of task $i$ in the direction $\mathbf{v}/\|\mathbf{v}\| \in \mathbb{R}^d$ is inversely related to $\mathbf{v}^\top \mathbf{\Sigma}_i \mathbf{v}/\|\mathbf{v}\|^2$. {\em In summary, a large variance in  $\mathbf{\Sigma}_i$ along all directions corresponds to easy tasks, and likewise a small variance corresponds to hard tasks.}

% {\em (ii) (Intuition on $\mathcal{E}_m(\mathbf{w}_{MAML}^\ast)$ vs $ \mathcal{E}_m(\mathbf{w}_{NAL}^\ast)$)}  



% This structure derives from the fact that both $\mathbf{w}_{MAML}^\ast$ and $\mathbf{w}_{NAL}^\ast$ are
% %in the set of normalized sums of nonnegative matrix transformations of the $\mathbf{w}_i^\ast$'s. 
% %This implies that they are 
% in the convex hull of the task optimal solutions $\mathbf{w}_i^\ast$.

%We conjecture that the same argument holds for $d>1$.
% note that the feasible set for this optimization problem corresponds to w in the convex hull of the training tasks, not all of Rd. But this is fine because 

% One can show that the optimal weights are proportional to the inducing matrix, because this best balances the distances. Consider the scalar case in with two tasks (i.e. $d=1$ and $T=2$). Here, the excess risks are of the form... Balancing the distances makes sense from an optimization standpoint... {\em }


%Consider the optimization problem
%\begin{align}
 %   &\min_{a}a^\top (\sum_{i=1}^T b_i c_i c_i^\top) a  \nonumber \\
  %  &\text{s.t.} \quad a \in \Delta_T \nonumber
%\end{align}
%The $c_i$'s are not orthogonal:
%\begin{align}
 %   c_i^\top c_{i'} = \sum_{j = 1}^T (w^\ast_{j,k} - w^\ast_{i,k})(w^\ast_{j,k} - w^\ast_{i',k}) \neq^\ast 0
%\end{align}
%but they are linearly independent if no two points are co-located

%Rayliegh quotient problem with l1 norm constraint, if eigenvector corresponding to max eigenvalue of matrix is nonnegative, then that eigenvector is the solution. We expect $b$ to be the eigenvector with the largest eigenvalue, since the $a$ for MAML should be optimal and is proportional to $b$

%what are the eigenvectors of this?
%\begin{align}
%    (\sum_{i=1}^T b_i c_i c_i^\top) b = \left[\sum_i \sum_j  b_i c_{i,1} c_{i,j} b_j ,...,\sum_i \sum_j  b_i c_{i,T} c_{i,j} b_j \right]^\top
%\end{align}
%...$b$ is not necessarily an eigenvector

%induced norm


% {\em (iii) (Intuition $\mathbf{w}_{MAML}$ vs $\mathbf{w}_{NAL}$)}

% To gain intuition for this result we must analyze the role of task hardness. 
% Recall that task hardness depends on how quickly gradient descent can traverse the loss function of the task, with harder tasks requiring more steps of gradient descent to reach an optimal solution.  Since the loss functions $f_i$ are strongly convex, the rate with which gradient descent traverses each $f_i$ depends on 
% % the steepness of $f_i$, which in turn is determined by 
% the minimum eigenvalue of the Hessian of $f_i$, which is $\mathbf{\Sigma}_i$ in this setting.
% So, assume that the easy tasks have data with large variance in all directions (all the eigenvalues of their $\mathbf{\Sigma}_i$ are large), while the hard tasks have data with small variance in all directions (all the eigenvalues of their $\mathbf{\Sigma}_i$ are small). 

% Suppose that the task environment has only easy and hard tasks that occur with equal probability.

% Note that both $\mathbf{w}_{MAML}^\ast$ and $\mathbf{w}_{NAL}^\ast$ are normalized weighted sums of the task optimal solutions. For simplicity, consider the case in which $m$ and $n_2$ are large, thus the $\mathbf{Q}_i$ matrices are dominated by $\mathbf{\Sigma}_i(\mathbf{I}_d -\alpha \mathbf{\Sigma}_i)^2$. 

It is most helpful to interpret the solutions $\mathbf{w}_{MAML}^\ast$ and $\mathbf{w}_{NAL}^\ast$ and their corresponding excess risks through the lens of task hardness.
In this strongly convex setting, we naturally define \textbf{task hardness as the rate at which gradient descent converges to the optimal solution for the task}, with harder tasks requiring more steps of gradient descent to reach an optimal solution. For step size $\alpha$ fixed across all tasks, the rate with which gradient descent traverses each $f_i$ is determined by
% the steepness of $f_i$, which in turn is determined by 
the minimum eigenvalue of the Hessian of $f_i$, namely $\lambda_{\min}(\mathbf{\Sigma}_i)$.
So, for ease of interpretation, we can think of the easy tasks as having data with large variance in all directions (all the eigenvalues of their $\mathbf{\Sigma}_i$ are large), while the hard tasks have data with small variance in all directions (all $\lambda(\mathbf{\Sigma}_i)$ are small). 

Note that both $\mathbf{w}_{MAML}^\ast$ and $\mathbf{w}_{NAL}^\ast$ are normalized weighted sums of the task optimal solutions, with weights being functions of the $\mathbf{\Sigma}_{i}$'s.
For simplicity, consider the case in which $m$ and $n_2$ are large, thus the $\mathbf{Q}_i$ matrices are dominated by $\mathbf{\Sigma}_i(\mathbf{I}_d -\alpha \mathbf{\Sigma}_i)^2$. 
% Further, assume that the task environment has only easy and hard tasks that occur with equal probability.
Since the weights for $\mathbf{w}_{NAL}^\ast$ are proportional to the $\mathbf{\Sigma}_i$ matrices, $\mathbf{w}_{NAL}^\ast$ \textbf{is closer to the easy task optimal solutions}, as $\mathbf{\Sigma}_i$ has  large energy for easy tasks and small energy for hard tasks. Conversely, the MAML weights are determined by $\mathbf{\Sigma}_i(\mathbf{I}_d - \alpha \mathbf{\Sigma}_i)^2$, which induces a relatively larger weight on the hard tasks, 
% since the spectrum of $(\mathbf{I}_d - \alpha \mathbf{\Sigma}_i)^2$ is small for the easy tasks, 
so $\mathbf{w}_{MAML}^\ast$  \textbf{is closer to the hard task optimal solutions}. 

Note that easy tasks can be approximately solved after one step of gradient descent from far away, which is not true for hard tasks.  We therefore expect (I) MAML to perform well on both hard and easy tasks since $\mathbf{w}_{MAML}^\ast$ is closer to the optimal solutions of hard tasks, and (II) NAL to perform well on easy tasks but struggle on hard tasks since $\mathbf{w}_{NAL}^\ast$ is closer to the optimal solutions of easy tasks.
We explicitly compute the excess risks of $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ as follows.
\begin{proposition} \label{er}
The excess risks for $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ are:
%\sim p(\mathcal{T})
\begin{align} 
\mathcal{E}_m(\mathbf{w}_{NAL}^\ast) &= \tfrac{1}{2} \mathbb{E}_{i} \Big\| \mathbb{E}_{i'}\big[\mathbf{\Sigma}_{i'}\big]^{-1} \mathbb{E}_{i'}\big[\mathbf{\Sigma}_{i'} (\mathbf{w}_{i'}^\ast\! -\! \mathbf{w}_{i}^\ast)\big]  \Big\|_{\mathbf{Q}_i^{(m)}}^2 \label{erm_loss} \\
\mathcal{E}_m(\mathbf{w}_{MAML}^\ast)
&= \tfrac{1}{2} \mathbb{E}_{i} \Big\| \mathbb{E}_{i'}\big[\mathbf{Q}_{i'}^{(n_2)}\big]^{-1}   \mathbb{E}_{i'}\big[\mathbf{Q}_{i'}^{(n_2)} (\mathbf{w}_{i'}^\ast - \mathbf{w}_{i}^\ast)\big]  \Big\|_{\mathbf{Q}_i^{(m)}}^2\!\! \label{multitask-fin-maml}
\end{align}
\end{proposition}
We next formally interpret these excess risks, and develop intuitions (I) and (II), by focusing on two key properties of the task environment: task hardness discrepancy and task geography.


\subsection{Hardness discrepancy}
\label{section:hardness}


%We will explore the relationship between both of these parameters in the next two subsections, giving insights regarding the sample sizes along the way.
% Here we empirically analyze the effects of task hardness on the relative performance of NAL and MAML by running simulations with varying task data covariance matrices.
% To isolate these effects, we consider a simple setting with $T=2$ tasks in $d=10$ dimensions. %\footnote{The excess risks $\mathcal{E}(\mathbf{w}_{NAL}^\ast)$ and $\mathcal{E}(\mathbf{w}_{MAML}^\ast)$ can be decomposed as the sum of the excess risks in each dimension, so the total excess risks in high dimensional settings are just summations of the low-dimensional excess risks, justifying our consideration of the low-dimensional case.}.
%To clarify notation, $\lambda_{i,k}$ is the variance of the data for the $i$-th task in the $k$-th dimension.

We analyze the levels of task hardness that confer a significant advantage for MAML over NAL in this section.
To do so, we compare $\mathbf{w}_{MAML}^\ast$ and $\mathbf{w}_{NAL}^\ast$ in an environment with two tasks of varying hardness. 
% simulate an environment with two tasks of varying hardness, and compare the MAML and NAL solutions. 
We let $n_2\!=\!m$, $\mathbf{\Sigma}_1\!=\!\rho_H \mathbf{I}_d$, and $\mathbf{\Sigma}_2\!=\!\rho_E\mathbf{I}_d$, where $\rho_{H}\!<\!\rho_E$, thus task 1 is the hard task.{\footnote{The effects of task hardness could be removed by scaling the data so that it would have covariance $\alpha^{-1}\mathbf{I}_d$. However, the current setting is useful to build intuition. Further, one can imagine a similar setting in which the first dimension has variance $\alpha^{-1}$ and the rest have variance $\rho_{H}$, in which scaling would not be possible (as it would result in gradient descent not converging in the first coordinate).
}} 
% . We fix $\rho_E=1$ and vary $\rho_H$ in $(0,1]$, thus task 1 is the hard task for all values of $\rho_H<1$.
%investigate how $\mathcal{E}(\mathbf{w}_{NAL})$ and $\mathcal{E}(\mathbf{w}_{MAML})$ change with the variance of the task 1 data, which we hold constant at $\nu$ in both dimensions (thus $\mathbf{\Sigma}_1 = \nu \mathbf{I}_d$).



% \begin{figure}[t]
% \vskip -0.1in
% \begin{center}
% \centerline{\hspace{8mm}\includegraphics[width=0.9\columnwidth]{fig3.pdf}}
% \vspace{-2mm}
% \caption{First coordinates of the empirical solutions $\mathbf{w}_{NAL}$ and $\mathbf{w}_{MAML}$ and their asymptotic analogues $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$  (top row) and the corresponding excess risks (bottom row). For the empirical values, 95\% confidence intervals are given. %over 5 trials
% }
% \label{fig:11}
% \end{center}
% \end{figure}



% For each value of $\rho_H$ and $m$, the empirical solutions are found by running SGD on the NAL and MAML training objectives given in (\ref{emp_orig}) and (\ref{emp_maml}), respectively, and their excess risks are estimated empirically. 
% On each iteration, we sample $n_1+n_2$ labelled points from each task, where $n_1=25$ and $n_2=m$ vary across the three columns in Figure \ref{fig:1}. 
% After 2000 iterations, we estimate the excess risks of the final iterates $w_{NAL}$ and $w_{MAML}$ by sampling 3000 task instances with $m$ labelled samples used for the SGD update. 
% The theoretical values are given by equations 
% \eqref{maml_pop}, \eqref{erm_loss} and \eqref{multitask-fin-maml}.
% \ref{thm:converge} and \ref{thm:convergeMAML} and Proposition \ref{er}.
In this setting, the NAL and MAML solutions defined in (\ref{maml_pop}) can be simplified as \begin{align}\mathbf{w}^\ast_{NAL} = \frac{\rho_H}{\rho_H + \rho_E} \mathbf{w}_{1}^\ast + \frac{\rho_E}{\rho_H + \rho_E} \mathbf{w}_{2}^\ast, \qquad \mathbf{w}_{MAML}^\ast = \frac{a_H}{a_H + a_E} \mathbf{w}_{1}^\ast + \frac{a_E}{a_H + a_E} \mathbf{w}_{2}^\ast,\end{align}
where $a_E \coloneqq (\rho_E(1 - \alpha \rho_E)^2 +\frac{d+1}{m}\alpha^2\rho_E^3)$ and $a_H \coloneqq (\rho_H(1 - 
\alpha\rho_H)^2 +\frac{d+1 }{m}\alpha^2 \rho_H^3)$. 
Note that the natural choice of $\alpha$ is the inverse of the largest task smoothness parameter ($\frac{1}{\rho_E}$ in this case). Setting $\alpha = \frac{1}{\rho_E}$ yields $a_E = \frac{d+1}{m}\rho_E$ and $a_H = \rho_H(1 - 
\frac{\rho_H}{\rho_E})^2 +\frac{(d+1) \rho_H^3 }{m \rho_E^3}$. As a result, we can easily see that for sufficiently large values of $m$, we have $a_H > a_E$. This observation shows that the solution of MAML is closer to the solution of the harder task, i.e., $\mathbf{w}_1^*$. On the other hand, $\mathbf{w}_{NAL}$ is closer to $\mathbf{w}_{2}^*$, the solution to the easy task, since $\rho_H < \rho_E$.
% Thus, unlike in single-task learning, the convergence rate for SGD depends on the ratio of the task's  strong convexity parameter to the maximum task smoothness parameter,   not on the condition number for the task.

% Note that $\mathbf{w}_{NAL}$ is closer to $\mathbf{w}_{2}^*$, the solution to the easy task, since $\rho_H < \rho_E$. On the other hand, for large values of $m$, we have $a_H\approx \rho_H(1 - \alpha \rho_H)^2$ and $a_E \approx \rho_E (1 - \alpha \rho_E)^2$, and as a result $a_H>a_E$ since $(1 - \alpha \rho_E)^2$ is zero by choice of . 

Considering these facts, we expect the performance of MAML solution after adaptation to exceed that of NAL. Using Proposition \ref{er}, the excess risks for NAL and MAML in this setting are 
\begin{align} \label{eer}
    \mathcal{E}_m(\mathbf{w}_{NAL}) = \frac{a_E \rho_H^2+ a_H \rho_E^2}{(\rho_E+ \rho_H)^2}, \quad \mathcal{E}_m(\mathbf{w}_{MAML}) = \frac{a_E a_H }{a_E+ a_H}.
\end{align}
Recalling that $a_E\approx 0$ for $m\gg d$, we conclude that MAML achieves near-zero excess risk in the case of large $m$. In particular, we require that ${\rho_H}(1- \frac{\rho_H}{\rho_E})^2 \gg \frac{d\rho_E}{m}$, otherwise the $O(d/m)$ terms in $a_E$ and $a_H$ are non-negligible. Meanwhile, for NAL we have $\mathcal{E}_m(\mathbf{w}_{NAL}) =  \frac{a_H \rho_E^2 }{(\rho_E+ \rho_H)^2}$, which may be significantly larger than zero if $\frac{\rho_H}{\rho_E} \ll 1$, i.e. the harder task is significantly harder than the easy task. Importantly, the error for NAL is dominated by poor performance on the hard task, which MAML avoids by initializing close to the hard task solution.
Thus, these expressions pinpoint the level of hardness discrepancy needed for superior MAML performance: {\em $\frac{\rho_H}{\rho_E}$ must be much smaller than 1, but also larger than 0, such that $\frac{\rho_H}{\rho_E}(1- \frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$.} 

% Importantly, the error for NAL is solely due to poor performance on the hard task, which MAML avoids by initializing close to the hard task solution.
% and is solely due to error on the hard task. Thus, MAML 
% Thus, MAML achieves small excess risk by initializing close to the solution of the hard task, 


 \begin{figure*}[t]
% \vskip -0.1in
\begin{center}
%\centerline{\includegraphics[width=0.9\textwidth, height=3.9cm]{intro2.png}}
% for aistats 2 column, it was 0.21\textwidth
% **** FOR NEURIPS, IT WAS 0.255 *****
     \begin{subfigure}[b]{0.263\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/twotasks_loc_2000t.pdf}
         \caption{}
         \label{fig:y equals x}
     \end{subfigure}
    %  \hfill
    \hspace{-4mm}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/twotasks_er_2000t.pdf}
         \caption{}
         \label{fig:three sin x}
     \end{subfigure}
    %  \hfill
    \hspace{1mm}
     \begin{subfigure}[b]{0.263\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/twotasks_loc_100t.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
    %  \hfill
    \hspace{-4mm}
     \begin{subfigure}[b]{0.23\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/fig2_4.pdf}
         \includegraphics[width=\textwidth]{NeurIPS/twotasks_er_100t.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
     \vspace{-2mm}
        \caption{First coordinates of $\mathbf{w}_{MAML}^\ast$, $\mathbf{w}_{NAL}^\ast$ and their excess risks for various $\rho_H$ for large $m$ (in subplots (a)-(b) for $m\!=\!2000$) and small $m$  (in subplots (c)-(d) for $m\!=\!100$).}
        \label{fig:three graphs}
%\caption{Excess risks and optimal solutions for MAML and NAL in various types of task environments.}
 \vspace{-2mm}
\label{fig:11}
\end{center}
% \vskip -0.1in
\end{figure*}


Figure \ref{fig:11} visualizes these intuitions in the case that $\mathbf{w}_1^\ast = \mathbf{1}_d$, $\mathbf{w}_2^\ast = -\mathbf{1}_d$, $d=10$ and $\sigma^2= 0.01$. Subfigures (a) and (c) show the locations of the first coordinates of $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ for varying $\rho_H$, and $m=2000$ and $m=500$, respectively. Subfigures (b) and (d) show the corresponding excess risks. We observe that unlike NAL, MAML initializes closer to the optimal solution of the harder task as long as $\frac{\rho_H}{\rho_E}$ is not close to zero or one, which results in significantly smaller excess risk for MAML compared to NAL in such cases, especially for large $m$. 


Figure \ref{fig:11} further shows that the MAML and NAL excess risks go to zero with $\rho_H$. This is also shown in (\ref{eer}) and the definition of $a_H$, and points to the fact that {\em too} much hardness discrepancy causes no gain for MAML. The reason for this is that $\rho_H\!\rightarrow\!0$ corresponds to the hard task data going to zero (its mean), in which case any linear predictor has negligible excess risk. Consequently, both NAL and MAML ignore the hard task and initialize at the easy task to achieve near-zero excess risk here.

% {\color{red} Need to discuss $\frac{\rho_H}{\rho_E}(1- \frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$ condition somewhere in here I think}

% $(1 - \alpha \rho_E)^2$ is zero so we have $a_E < a_H$ for large $m$. As a result, the solution of MAML is closer to the solution of the harder task.

% The top row of Figure \ref{fig:11} shows the first coordinates of the population-optimal solutions for NAL and MAML, as well as the task optimal solutions, for varying $\rho_H$ and $m$. The bottom row shows the corresponding excess risks for the NAL and MAML solutions. 



% \begin{figure*}[t]
% \vskip -0.1in
% \begin{center}
% \centerline{\includegraphics[width=1.8\columnwidth]{ratios1.png}}
% \vspace{-2mm}
% \caption{Excess risks for both NAL and MAML and the ratios of the NAL excess risk to the MAML excess risk in the setting with half easy and half hard tasks. Empirical and theoretical versions are given for each quantity, and 95\% confidence intervals over 5 random trails are shown.
% }
% \label{fig:complex}
% \end{center}
% \vskip -0.2in
% \end{figure*}

%  \begin{figure}[htp]
% \vskip -0.1in
% \begin{center}
% %\centerline{\includegraphics[width=0.9\textwidth, height=3.9cm]{intro2.png}}
%     %  \hfill
%      \begin{subfloat}[]{}
%          \centering
%          \includegraphics[width=0.8\columnwidth]{ratio1.png}
%         %  \caption{$y=5/x$}
%          \label{fig:ratio1a}
%      \end{subfloat}
%     %  \hfill
%      \begin{subfloat}[]{}
%          \centering
%          \includegraphics[width=0.8\columnwidth]{ratio2.png}
%         %  \caption{$y=5/x$}
%          \label{fig:ratio2b}
%      \end{subfloat}
%      \vspace{-4mm}
%         \caption{Excess risks for both NAL and MAML and the ratios of the NAL excess risk to the MAML excess risk in the setting with half easy and half hard tasks. Empirical and theoretical versions are given for each quantity, and 95\% confidence intervals over 5 random trails are shown.}
%         \label{fig:ratio2}
% \vspace{-2mm}
% \label{fig:complex}
% \end{center}
% \vskip -0.1in
% \end{figure}




% . On each iteration, $n_1+n_2$ labelled samples are drawn randomly from each of the two tasks, with $n_1 = 25$ and $n_2=m$ varying across the three columns in Figure \ref{fig:1}. The gradient of the NAL objective is estimated using these samples, and $\mathbf{w}_{NAL}$ is updated via one step of SGD with tuned step size. For MAML, $n_2$ of the samples are used to compute a local set of parameters for each task via one step of SGD with step size $\alpha$. Then, the gradient of the task losses at these local parameters is estimated using the $n_1$ `outer' loop samples for each task, and $\mathbf{w}_{MAML}$ is updated with an SGD step using the average of these gradients. Note that this is a first-order approximation of MAML (FO-MAML, \cite{finn2017model}) since it ignores the Hessians of the task losses, but we will see that it still converges to the optimal solution of the MAML objective. After 2000 iterations, for each task, both  $\mathbf{w}_{NAL}$ and $\mathbf{w}_{MAML}$ are updated with one step of SGD with step size $\alpha$ using $m$ samples. These local parameters are then evaluated on 3000 test samples for each task, allowing for estimation of $\mathcal{E}_m$.

% The first coordinate of the empirical solutions $\mathbf{w}_{NAL}$ and $\mathbf{w}_{MAML}$ after 2000 iterations are plotted as functions of $\nu$ in the first row of Figure \ref{fig:1}, where each plot corresponds to a different setting of $n_2$ and $m$. The first coordinates of $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ in these settings are plotted as well. 

%The key takeaway from Figure \ref{fig:1} is that 
% The empirical results plotted in the top row of Figure \ref{fig:11} confirm our intuition that for $\rho_H$ sufficiently small, MAML initializes closer to the harder task, assuming large $m$. Further, we observe in the bottom row of Figure \ref{fig:11} that when $m \gg d$, {\em MAML substantially outperforms NAL for small $\rho_H$  by finding a solution that is closer to the solution of the harder task} (task~1). The largest gain for MAML is for $\rho_H \! \in \! [0.1,0.4]$. 
%matching our intuition from the previous section. 
%When the tasks are equally hard (i.e. $\rho_H =1 = \rho_E$), both NAL and MAML yield solutions halfway between the tasks. But 
%When the disparity between the hardness of the tasks is large, i.e. $\rho_H \ll 1$, $\mathbf{w}_{MAML}$ is closer to the optimal solution of the harder task (task 1), matching our intuition from the previous section. %Indeed, this makes sense because 
%. Since $n_2=m$ is large, the stochastic gradient has low variance, so the easy task can be solved by initializing from almost anywhere. 



% Given one step of SGD with a large number of samples, it makes sense to initialize closer to the solution of the harder task to improve performance on that task without sacrificing easy task performance, matching our previous intuition. %since the stochastic gradient has small variance. 
% Meanwhile, NAL does not account for the one step of SGD that may be executed at test time, and
% %does not account for the one step of SGD that may be used for fine-tuning at test time. Without this foresight, it 
% initializes closer to the optimal solution of the easy task because it has a steeper loss function, compromising hard task performance. 

\noindent \begin{remark} The condition $\frac{\rho_H}{\rho_E}(1- \frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$ requires that $m \gg d$. However, this condition arises due to the simplification $\text{tr}(\mathbf{\Sigma}_i)=O(d)$, where $\text{tr}(\mathbf{\Sigma}_i)$ can be thought of as the effective problem dimension \citep{kalan2020minimax}. In realistic settings, the effective dimension may be $o(d)$, which would reduce the complexity of $m$ accordingly.
%is due to the fact that $m$ must be large enough to solve the easy task in one SGD step from far away. However, $d$ truly scales with the effective problem dimension, which is reduced in low-rank scenarios \cite{kalan2020minimax}.
% This is captured by the term in the $\mathbf{Q}_{i}^{(m)}$ matrices that scales with $ \text{tr}(\mathbf{\Sigma}_i^2)$, which is closely related to the effective problem dimension \cite{kalan2020minimax}. 
% Since the dependence of $m$ on the problem dimension is not the focus of this paper, we set each $\mathbf{\Sigma}_i$ such that $\text{tr}(\mathbf{\Sigma}_i^2) = \Theta(d)$ throughout. 
\end{remark}



% \textbf{Complexity of $m$.} Note that MAML's advantage only holds for $m$ large enough
% %, i.e. the stochastic gradient is accurate enough, 
% to solve the easy task in one SGD step from far away, i.e. $m > d$. This is captured by the second term in the $\mathbf{Q}_{i}^{(m)}$ matrices, which scales with $\frac{\alpha^2 \text{tr}(\mathbf{\Sigma}_i^2)}{m} \mathbf{\Sigma}_i$. Note that the size of $m$ needed to make this term negligible depends on $\text{tr}(\mathbf{\Sigma}_i^2)$, which in turn is closely related to the effective problem dimension \cite{kalan2020minimax}. Thus, few fine-tuning samples are needed when the effective problem dimension is small. Since this is not the focus of this paper, we set each $\mathbf{\Sigma}_i$ such that $\text{tr}(\mathbf{\Sigma}_i^2) = \Theta(d)$ throughout.


% We have set the trace  $\text{tr}(\mathbf{\Sigma}_i^2)$ to scale with $d$, thereby necessitating $m =\Omega(d)$ to make this term negligible.  However, the trace  $\text{tr}(\mathbf{\Sigma}_i^2)$ can be thought of as the effective problem dimension for linear regression, which is often $o(d)$. Thus, the complexity of $m$ is decreases with smaller effective dimension. in most learning problems, the effective problem dimension is $o(d)$, which would reduce the complexity of $m$.


% The meta-test time benefits of initializing closer to the hard task are also dependent on the number of samples used in the inner gradient update. We plot the empirical excess risks, computed using the procedure described above, in the second row of Figure \ref{fig:1}. We also show the theoretical excess risks of the asymptotic NAL and MAML solutions. When $m$ is large, and $n_2$ is also large, then the MAML strategy of initializing closer to the harder task confers very small excess risk and a significant improvement over NAL. Conversely, when $m$ is small, the SGD update is too noisy for MAML to improve significantly over NAL. Also note that the middle three columns suggest that the ultimate setting of $n_2$ is $n_2=m$.


\subsection{Task geography}
\label{section:linear_experiments}


% \noindent \textbf{Setting.} 
The second important property of the task environment according to Proposition 1 is the location, i.e. geography, of the task optimal solutions. In this section, we study how task geography affects the  MAML and NAL excess risks by considering a task environment with many tasks. 
In particular, the task environment $\mu$ is a mixture over distributions of hard and easy tasks, with mixture weights $0.5$. The optimal solutions $\mathbf{w}_i^*\in  \mathbb{R}^d$ for hard tasks are sampled according to $\mathbf{w}_i^* \sim \mathcal{N}(R \mathbf{1}_d,r_H \mathbf{I}_d)$ and for easy tasks are sampled as $\mathbf{w}_i^* \sim \mathcal{N}( \mathbf{0}_d,r_E \mathbf{I}_d)$. Therefore $R$ is the dimension-normalized distance between the centers of the hard and easy tasks' optimal solutions, and $r_H$ and $r_E$ capture the spread of the hard and easy tasks' optimal solutions, respectively.
The data covariance is $\mathbf{\Sigma}_i=\rho_H \mathbf{I}_d$ for the hard tasks and $\mathbf{\Sigma}_i=\rho_E \mathbf{I}_d$ for the easy tasks, recalling that $\rho_H$ and $\rho_E$ parameterize hardness, with smaller $\rho_H$ meaning  harder task. In this setting the following corollary follows from Proposition \ref{er}.
\begin{corollary} \label{prop2}
In the setting described above, the excess risks of  $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ are:
     \begin{align}
    \mathcal{E}_m(\mathbf{w}_{NAL}^\ast)
    &=\tfrac{d}{4(\rho_E+\rho_H)^2} \Big[
    (a_E \rho_E^2 + 2 a_E \rho_E \rho_H)r_E + a_E \rho_H^2 (r_E + R^2) \nonumber \\
    &\quad\quad\quad\quad\quad\quad + (a_H \rho_H^2 + 2 a_H \rho_E \rho_H)r_H
      + a_H \rho_E^2 (r_H + R^2) \Big]\label{erm_excess_eh} \\
   \mathcal{E}_m(\mathbf{w}_{MAML}^\ast) &=\tfrac{d}{4(a_E+a_H)^2} \Big[
    (a_E^3 + 2 a_E^2 a_H)r_E  + (a_H^3 + 2 a_E a_H^2)r_H \nonumber \\
    &\quad\quad\quad\quad\quad\quad + a_E a_H^2 (r_E + R^2) +  a_E^2 a_H (r_H + R^2) \Big] \label{maml_excess_eh}
    \vspace{-2mm}
     \end{align}
     \vspace{-2mm}
where $a_E \coloneqq \rho_E(1 - \alpha \rho_E)^2 +\frac{d+1}{m}\alpha^2\rho_E^3$ and $a_H \coloneqq \rho_H(1 - 
\alpha\rho_H)^2 +\frac{d+1 }{m}\alpha^2 \rho_H^3$. 
\end{corollary}
% sample complexity dependence on m is very poor.... why: because the functions are convex.... if at test time you have a noisy gradient....  what can you do..characterize gradient variance.... 
% should be able to show some improvement as long as the gradient is somewhat informative....choose step size proportional to m?

% Note that the coefficients of the displacement metrics in the NAL excess risk
% sum to the same value for both the MAML and NAL excess risks. %, which can be easily seen by observing 
%that the NAL coefficients 
%are a permutation of the MAML coefficients.  
% So, the comparison between the excess risks for MAML and NAL depends entirely on which displacement metrics each algorithm weighs more than others in its excess risk function.
% For large $m$ and large $\rho_E$ %(i.e., large disparity in the difficulty of the hard and easy tasks), 
% the coefficient of $D_{HH}$ is dominant for the MAML excess risk, and the coefficient of $D_{HE}$ is dominant for the NAL excess risk. These observations are summarized in the following result.

%To do so, we first simplify the setting by assuming that $\rho_E + \rho_H=1 = \alpha$, thus we can substitute $1-\rho_H$ for $\rho_E$. We also assume that there is no noise whatsoever, i.e. $m \rightarrow \infty$. We compare the coefficients for each of the displacement terms in this setting for MAML and NAL below, starting with MAML:
% \begin{align*}
%     C_{D_{EE}} = \rho_H^4(1-\rho_H)/2T, &\quad C_{D_{HH}} = \rho_H(1-\rho_H)^4/2T, \nonumber \\
%     C_{D_{EH}} = \rho_H^2(1-\rho_H)^3/2T, &\quad C_{D_{E,EH}} = 2 \rho_H^3(1-\rho_H)^2/2T, \nonumber \\
%     C_{D_{HE}} = \rho_H^3(1-\rho_H)^2/2T, &\quad C_{D_{H,EH}} = 2\rho_H^2(1-\rho_H)^3/2T
% \end{align*}
% Since by definition $\rho_H <0.5$, we see that for MAML, $C_{D_{HH}} > C_{D_{H,EH}} > C_{D_{EH}} > C_{D_{E,EH}}  > C_{D_{HE}} > C_{D_{EE}}$%, where the coefficients differ typically by a factor of $\rho_H/(1-\rho_H)$. 
% This shows that the MAML error depends heavily on the compactness of the hard task locations, while depending very little on the compactness of the easy task locations.

% The coefficients for NAL are as follows:
% \begin{align*}
%     C_{D_{EE}} = \rho_H^2(1-\rho_H)^3, &\quad  C_{D_{HH}} =  \rho_H^3(1-\rho_H)^2, \nonumber \\
%     C_{D_{EH}} =  \rho_H^4(1-\rho_H), &\quad  C_{D_{E,EH}} = 2 \rho_H^3 (1-\rho_H)^2, \nonumber \\              
%     C_{D_{HE}} =  \rho_H(1-\rho_H)^4, &\quad C_{D_{H,EH}} = 2 \rho_H^2 (1-\rho_H)^3 
% \end{align*}
% For NAL, we have  $C_{D_{HE}} > C_{D_{H,EH}} > C_{D_{EE}} > C_{D_{E,EH}}  > C_{D_{HH}} > C_{D_{EH}}$, as expected. Thus the NAL error depends heavily on the extent to which the hard tasks are in the center of the easy tasks (captured by $D_{HE}$). These observations tell us that the key difference between MAML and NAL is that the MAML error depends most on $D_{HH}$, while the NAL error depends most on  $D_{HE}$. 

% We can formalize these insights in the following theorem:
% \begin{corollary} \label{prop3}
% {\color{red} Old} In the setting described in Theorem 1, with the additional assumptions that $m \rightarrow \infty$, $\rho_E = 1 - \rho_H$ and all error terms with at least quadratic dependence on $\rho_H$ are negligible, 
% the relative empirical excess risk for NAL compared to MAML is bounded as:
% %\begin{align}
%   %\frac{(1-\rho_H)^3 D_{HE}}{(1-\rho_H)^3 D_{HH} + O(\rho_H)} \leq \frac{f({w_{NAL}})}{f(w_{MAML})} \leq  \frac{(1-\rho_H)^3 D_{HE}+ O(\rho_H)}{(1-\rho_H)^3 D_{HH} } 
%   $\frac{\mathcal{E}_\infty(\mathbf{w}_{NAL})}{\mathcal{E}_\infty(\mathbf{w}_{MAML})}= \Theta\big( \frac{D_{HE}}{D_{HH}} \big)$
%   \end{corollary}
Each excess risk is a normalized weighted sum of the quantities $r_E, r_H$ and $R^2$. So, the comparison between MAML and NAL depends on the relative weights each algorithm induces on these task environment properties. If $\frac{\rho_H}{\rho_E}(1-\frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$, then $a_H\gg a_E$ and the dominant weight in $\mathcal{E}_m(\mathbf{w}_{MAML}^\ast)$ is on the $r_H$ term, 
while the dominant weights in $\mathcal{E}_m(\mathbf{w}_{NAL}^\ast)$ are on the $r_H + R^2$ and $r_H$ terms. This observation leads us to obtain the following corollary of Proposition \ref{er}.
%This suggests that the gain for MAML over NAL depends on $R^2/r_H$, which is shown in the following result.
\begin{corollary} \label{prop3}
In the above setting, with $\alpha = 1/\rho_E$ and $\frac{\rho_H}{\rho_E}(1-\frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$,
the relative excess risk for NAL compared to MAML satisfies
 \vspace{-2mm}
\begin{align}
    \frac{\mathcal{E}_m(\mathbf{w}_{NAL}^\ast)}{\mathcal{E}_m(\mathbf{w}_{MAML}^\ast)} \approx 1+\frac{ R^2}{ r_H}.
 \end{align}  
 \vspace{-1mm}
% Alternatively, in the limit as $m \rightarrow \infty$, $\rho_E \rightarrow 1$, and $\rho_H \rightarrow 0$, we have
% the relative excess risk for NAL compared to MAML is:
% \begin{align}
%   \lim_{m \rightarrow \infty, \rho_E \rightarrow 1, \rho_H \rightarrow 0}\frac{\mathcal{E}_m(\mathbf{w}_{NAL})}{\mathcal{E}_m(\mathbf{w}_{MAML})}= 1 + \frac{R^2}{r_H}
%  \end{align} 
%Numerically, we find that we need $m > d/\rho_H$ in order to realize the above asymptotic behavior.
\end{corollary}
 \vspace{-3mm}
Corollary \ref{prop3} shows  that MAML achieves large gain over NAL when: {\em (i) the hard tasks' solutions are closely packed} ($r_H$ is small) and  {\em (ii) the hard tasks' solutions are far from the center of the easy tasks' solutions} ($R$ is large). Condition (i) allows MAML to achieve a small excess risk by initializing in the center of the hard task optimal solutions, while condition (ii) causes NAL to struggle on the hard tasks since it initializes close to the easy tasks' solutions. These conditions are reflected by the fact that the MAML excess risk weighs $r_H$ (the spread of the hard tasks) most heavily, whereas the NAL excess risk puts the most weight on $R^2$ (distance between hard and easy task solutions) as well as $r_H$.

Note that the above discussion holds under the condition that $a_H \gg a_E$. In order for $a_H \gg a_E$, we must have $\frac{\rho_H}{\rho_E}(1-\frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$, i.e. $m\gg d$ and $0 < \frac{\rho_H}{\rho_E} \ll 1$, as we observed in our discussion on hardness discrepancy. Now, we see that even with appropriate hardness discrepancy, the hard tasks must be both closely packed and far from the center of the easy tasks in order for MAML to achieve significant gain over NAL. This conclusion adds greater nuance to prior results \citep{balcan2019provable,jose2021information}, in which the authors argued that gradient-based meta-learning (e.g. MAML) is only effective when all of the tasks' optimal solutions are close to each other (in our case, all of $r_E$, $r_H$ and $R$ are small). 
Crucially, our analysis shows that NAL would also perform well in this scenario, and neither $r_E$ nor $R$ need to be small for MAML to achieve small excess risk.

%, and our analysis shows that the easy tasks must be far from the hard tasks in order for NAL to perform poorly, and only the hard tasks need to be closely packed for MAML to perform well.


% We consider a setting in which all of the tasks are either easy (well-conditioned) or hard (poorly conditioned). Let $E$ and $H$ denote the sets of easy and hard tasks, respectively. For all $i \in E$, $\sigma_{\min}(\mathbf{\Sigma}_i) = 0.9$, and for all $i \in H$, $\sigma_{\min}(\mathbf{\Sigma}_i) = 0.1$. In Figure \ref{fig:eh_geo2}, we plot the values of the excess risks (\ref{erm_loss}) and (\ref{multitask-fin-maml}) for four distinct task environments. 
% %(\ref{maml_excess_eh}) and (\ref{erm_excess_eh})
% Since our focus for now is not on the effects of noise, we set $m=100$ to be relatively large. The easy and hard task optimal solutions are each sampled from multivariate normal distributions, which differ across task environments. For example, the leftmost column of \ref{fig:eh_geo2} shows the case when the easy and hard tasks are both closely packed, i.e. drawn from distributions with small variance, and have the same mean (only two dimensions are shown, but the task optimal solutions are distributed identically in all dimensions, so two dimensions are representative). In this case, both NAL and MAML have very small excess risk. In the second column, the hard tasks are spread out and have mean far from the mean of the easy tasks. Here, MAML outperforms NAL, but still has a very large error due to the dispersion of the hard tasks. 



To further explain these insights, we return to Figure \ref{fig:eh_geo_gen} in which easy and hard task optimal solutions are each sampled from $10$-dimensional Gaussian distributions of the form described above, and 100 random task optimal solutions are shown, along with the population-optimal MAML and NAL solutions. In subfigures (b), (c) and (d), we set $\rho_E = 0.9$, $\rho_H = 0.1$, and $m = 500$. Among these plots, the largest gain for MAML is in the case that the hard tasks' optimal solutions are closely packed (small $r_H$), and their centers are far from each other (large $R$), 
% as expected. The second-largest gain comes under the same conditions but with large $r_E$, 
{\em demonstrating the the primary dependence of relative performance on $R^2/r_H$.} 

We plot more thorough results for this setting in Figure \ref{fig:complex}. Here, we vary $R$ and compare the performance of $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ in settings with relatively large $r_H$ and small $r_E$, specifically choosing $r_H$ and $r_E$ such that $\frac{R^2}{r_H}\!=\!0.5$ and $\frac{R^2}{r_E}\!=\!10$ in (a)-(b), and $\frac{R^2}{r_H}\!=\!10$ and $\frac{R^2}{r_E}\!=\!0.5$ in (c)-(d). %As in Figure \ref{}
% We scale $r_H$ and $r_E$ with $R^2$ in order to highlight the asymptotic linear dependence of the ratio of the NAL excess risk to the MAML excess risk on $R^2/r_H$. 
Here we also plot the empirical solutions $\mathbf{w}_{NAL}$ and $\mathbf{w}_{MAML}$. 
% for $T\!=\!5000$, $\tau\!=\!1$, $n\!=\!600$ and $n_1\!=\!100$.
%by running SGD on the MAML and NAL objectives for 5000 iterations (details in Appendix \ref{app:}). % for $T=5000, \tau=1, n=600$ and $n_1=100$.
\begin{comment}
We also compare the population-optimal and empirical performance for both algorithms.
with empirical solutions $\mathbf{w}_{MAML}$ and ... found by running 5000 iterations of SGD with one task sampled per iteration.
\end{comment}
%For theoretical performance we directly plot the excess risks given in (\ref{maml_excess_eh}) and (\ref{erm_excess_eh}). 
%For empirical performance, we run SGD on the MAML and NAL objectives for 5000 iterations, then evaluate the resulting solution on 100 new tasks to compute the empirical excess risk $\hat{\mathcal{E}}_m$. 
{\em Again, MAML significantly outperforms NAL when $R^2/r_H$ is large (subfigures (c)-(d)), but not otherwise}.

% \begin{figure}
% \centering
%   \begin{subfigure}[b]{\columnwidth}
%   \centering
%     \includegraphics[width=0.7\columnwidth]{fig23.pdf} %make height=3cm for aistats version
%     % \vspace{-6mm}
%     \caption{$r_H =2R^2$, $r_E = 0.1R^2$}
%     % \vspace{2mm}
%     \label{fig:111}
%   \end{subfigure}
% %   \hfill %%
%   \begin{subfigure}[b]{\columnwidth}
%   \centering
%     \includegraphics[width=0.7\columnwidth]{fig21.pdf} %make height=3cm for aistats version
%     % \vspace{-6mm}
%     \caption{$r_H =0.1R^2$, $r_E = 2R^2$}
%     % \vspace{2mm}
%     \label{fig:222}
%   \end{subfigure}
%   \vspace{-4mm}
%   \caption{Excess risks for NAL and MAML and ratios of the NAL to MAML excess risk in the setting described in Section \ref{section:linear_experiments}. Empirical and theoretical versions are given for each quantity, with 95\% confidence intervals over 5 trials. The gain for MAML over NAL is significantly larger when $r_H$ is small, as in (a).
%   }
%   \label{fig:complex}
% \end{figure}


 \begin{figure*}[t]
% \vskip -0.1in
\begin{center}\begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/r0.pdf}
         \caption{$\frac{R^2}{r_H}\!=\!0.5,\; \frac{R^2}{r_E}\!=\!10$} %$r_H\!=\!2R^2$, $r_E\!=\!0.1R^2$
         \label{fig:five over x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
        %  \includegraphics[width=\textwidth,height=2.6cm]{NeurIPS/fig22.pdf}
         \includegraphics[width=\textwidth]{NeurIPS/ratio_0.pdf}
         \caption{$\frac{R^2}{r_H}\!=\!0.5,\; \frac{R^2}{r_E}\!=\!10$} %$r_H\!=\!2R^2$, $r_E\!=\!0.1R^2$
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/R1.pdf}
         \caption{$\frac{R^2}{r_H}\!=\!10,\; \frac{R^2}{r_E}\!=\!0.5$} %$r_H\!=\!0.1R^2$, $r_E\!=\!2R^2$
         \label{fig:y equals x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/ratio_1.pdf}
        %  \caption{$r_H\!=\!0.1R^2$, $r_E\!=\!2R^2$}
        \caption{$\frac{R^2}{r_H}\!=\!10,\; \frac{R^2}{r_E}\!=\!0.5$}
         \label{fig:three sin x}
     \end{subfigure}
        \caption{Theoretical and empirical excess risks for NAL and MAML and ratios of the NAL to MAML excess risk in the setting described in Section \ref{section:linear_experiments}. 
        % Theoretical versions are given for each quantity, with 95\% confidence intervals. %over 5 trials
        % The gain for MAML over NAL is significantly larger when $r_H$ is small relative to $R^2$, as in (c)-(d). 
        }
\label{fig:complex}
\end{center}
\vskip -0.1in
\end{figure*}

==> NeurIPS/Introduction.tex <==
%!TEX root = main.tex
\section{Introduction}

Large-scale learning models have achieved remarkable successes in domains such as computer vision and reinforcement learning. However, their high performance has come at the cost of requiring huge amounts of data and computational resources for training, meaning  they cannot be trained from scratch every time they are deployed to solve a new task. Instead, they typically must undergo a single pre-training procedure, then be fine-tuned to solve new tasks in the wild.

% models that can quickly learn how to solve new tasks, with access to limited computational resources and data for that task, have been much harder to come by.
% An important challenge in machine learning is to develop models that learn how to adapt to solve a new task with limited data and computational resources. 

{\em Meta-learning} aims to  address this problem by extracting an inductive bias from a large set of pre-training, or meta-training, tasks that can be used to improve test-time adaptation.  {\em Model-agnostic meta-learning} (MAML) \citep{finn2017model}, one of the most popular meta-learning frameworks, formulates this inductive bias as an initial model for a few gradient-based fine-tuning steps. Given that for  the model can be fine-tuned on any meta-test task before evaluating its performance, MAML aims to learn the best initialization for fine-tuning among a set of meta-training tasks. 
To do so, it executes an episodic meta-training procedure in which the current initialization is adapted to specific tasks in an {\em inner loop}, then the initialization is updated in an {\em outer loop}. 
This procedure has led to impressive few-shot learning performance in many settings \citep{finn2017model,antoniou2018train}.


% Model-Agnostic Meta-Learning (MAML) \citep{finn2017model} provides a framework for training models to achieve this goal.  %It formalizes the goal of finding models that can quickly adapt to tasks drawn from some environment by considering fast adaptation as one or a small number of stochastic gradient descent steps. 
% Instead of the classical training method of finding the model that minimizes the average loss across tasks without accounting for any adaptation, MAML aims to find the optimal initial model given that a few stochastic gradient descent (SGD) steps can be performed on any new task. To do so, it executes an episodic meta-training procedure wherein each episode consists of an inner loop task-specific adaptation and an outer loop model update.
% %, i.e., 
% %to find the best model for solving tasks drawn from some distribution, knowing that the model may be adapted with a small number of gradient-based updates on any new task. 
% %%%%%% 
% This framework has grown in popularity by yielding models empirically shown to adapt quickly to new tasks in settings such as few-shot image classification and meta-reinforcement learning.

% trained using the classical method which lacks the inner loop adaptation phase, and which we refer to as Empirical Risk Minimization (ERM).
%% , in settings such as few-shot image classification and meta-reinforcement learning \citep{finn2017model, antoniou2018train, mendonca2019guided}.

%To solve the MAML objective, the MAML algorithm iteratively updates the initialization for gradient descent by backpropagating through the loss after one or more gradient descent steps on sampled meta-training tasks. This amounts to executing (stochastic) gradient descent on the meta-loss objective.
%This procedure has achieved noted empirical success in areas including few-shot classification, where each task is to classify unlabeled samples from a particular set of classes \cite{snell2017prototypical}, and federated learning, where each client's workload is considered a task \cite{fallah2020personalized}. 
% Although MAML has achieved impressive empirical results \citep{finn2017model,antoniou2018train}, 

However, 
in some settings MAML's inner loop adaptation and the second derivative calculations resulting thereof may not justify their added computational cost compared to traditional, no-inner-loop pre-training. 
% \citep{fallah2020convergence}. 
% instead of solving the ERM problem via gradient descent, %(or in the case of federated learning, FedAvg with one local update step), 
%% % Solving the MAML objective raises numerous optimization challenges, including: (i) computing Hessian matrices at each iteration, (ii) dealing with a potentially unbounded smoothness parameter, and (iii) only having access to stochastic gradients that are either biased or have large variance \citep{fallah2020convergence}.
%, and first-order approximations are erroneous and/or complicated to implement. %We would like to understand why and when MAML achieves significant gain over ERM in order to help determine when it is appropriate to use MAML. 
% rapid learning also happens in the early layers \cite{goerttler2021exploring}
Multiple works have suggested that MAML's few-shot learning performance may not drop when executing the inner loop adaptation for only a fraction of the model parameters \citep{raghu2019rapid, oh2020does} or, in some cases, by ignoring the inner loop altogether \citep{bai2020important, chen2019closer, chen2020new, tian2020rethinking, dhillon2019baseline}. Unfortunately, the underlying reasons for MAML's behavior are still not well-understood, making it difficult to determine when inner loop adaptation  during meta-training yields meaningful benefit. 
%bernacchia2021meta,
% So, to determine when the MAML inner loop updates are worth their extra cost, we must determine the task environments in which MAML achieves significant gain over ERM.
% This begs the following question:

% {\em When does MAML's inner loop update confer significant advantage in test time adaptation?}

% In this work, we aim to determine 
% % We refer to the meta-training method that lacks an inner loop as Non-Adaptive Learning (NAL), which is equivalent to the classical method of trying to minimize the average loss across tasks. 
% when  inner loop adaptation signficicantly helps performance by considering . it never hurts in terms of performance, but when does it significantly help? we study the task landscape.


In this work, we investigate when and why MAML's inner loop updates provide significant gain for meta-test time adaptation. To achieve this, we focus on how the meta-training loss landscape induced by the MAML objective affects adaptation performance compared to the loss landscape induced by the classical objective without inner loop adaptation, which we term the Non-Adaptive Learning (NAL) method. Notably, MAML should always perform at least as well as NAL because its meta-training procedure aligns with the meta-test time evaluation of performance after a few steps of task-specific SGD. Thus, our goals are to quantify the gain provided by MAML and determine the scenarios in which this gain is most significant. We start by studying the multi-task linear regression setting since it allows us to compare the exact solutions and excess risks for MAML and NAL. 
% We show that MAML induces a global optimization landscape with optimal solution closer to the optimal solutions of the hard tasks, where task hardness is defined as the rate at which gradient descent converges towards the optimal solution for the task.
% Meanwhile, the TNIL solution is close to the optimal solutions of the easy tasks. MAML thereby outperforms TNIL on the hard tasks without sacrificing easy task performance, since they can still be solved in a small number of gradient descent steps. 
In doing so, we obtain novel insights on how MAML deals with hard tasks differently than NAL, and show that MAML achieves significant gain over NAL only if certain conditions are satisfied relating to the hardness and geography of the tasks. These observations provide a new understanding of MAML that is distinct from the representation learning perspective considered in recent works \citep{raghu2019rapid, du2020few, tripuraneni2020provable}.
We then give theoretical and empirical evidence generalizing these insights to neural networks.



% we compare MAML with the standard training method that lacks an inner loop, which we term the Non-Adaptive Learning (TNIL) method. 

% More specifically, \cite{raghu2019rapid} gave empirical evidence suggesting that MAML's impressive few-shot learning performance is due to its ability to learn a high-quality feature representation, and that it does not need to update the parameters of the representation in the inner loop in order to achieve this. Moreover, many recent theoretical and empirical works have shown that training without an inner loop adaptation phase can also yield high-quality representations in settings with a large number of classes whose labels are held fixed and non-mutually exclusive throughout training. Thus, the representation learning paradigm provides little consensus on why and when MAML should be used as opposed to standard methods.


% {\color{red}
% Several recent works have studied the reasons for MAML's effectiveness from a representation learning perspective. Specifically, \cite{raghu2019rapid,kao2021maml} gave experimental evidence that MAML learns a shared representation among tasks during meta-training. However, theoretical analysis has shown that standard  multi-task formulations can leverage all samples across tasks to learn a ground-truth representation when it exists in the hypothesis class \citep{du2020few, saunshi2020sample, tripuraneni2020provable, saunshi2021representation}, while results showing that MAML learns a quality representation are lacking.  Thus, the representation learning paradigm provides little consensus on why and when MAML should be used as opposed to standard methods.

% % while other empirical works have shown that standard pre-training can learn good representations for few-shot image classification as long as a large classifier is used that  learns all classes simultaneously throughout training, rather than re-learning new, shuffled labels for every task.
% }


% insert formal definition of hardness? but include general definition (hard to formalize) or only the definition for linear case? where to insert it? also need to make more clear why the min singular value





% instead consider the agnostic regime in which there may not be a shared representation among the tasks. We aim to clearly determine the benefits of MAML's inner loop updates vs standard pre-training in a simple setting in which each task is a linear regression.

% Moreover, a series of experimental works have shown that standard pre-training plus fine-tuning can sometimes match or even exceed the performance of MAML.
% is often closely matched by applying the second-order MAML updates to only a fraction of the model parameters, and ERM updates to the other parameters \citep{raghu2019rapid, oh2020does}. 
% Other recent works have studied how learning the low-dimensional representation of linear regression tasks can reduce the sample complexity of a new task \citep{saunshi2020sample, du2020few, tripuraneni2020provable}, 
% but this line of work does not show any unique benefits of MAML or its gradient-based meta-learning variants for learning the representation or solving a new task once the representation is learned. Indeed, any algorithm that learns the representation solves a new task with the same sample complexity.
% Ultimately, we hope to start a discussion on  when and why it is important to take an adaptation step during training -- a question which the representation learning literature has yet to answer.


% points: 
% - success of maml is not fully explained by
% --- there is evidence that maml does not learn a representation, since:
% --- erm also learns good representations
% --- indeed, recents works have shown that algorithms without inner loops also perform well.

% \cite{goerttler2021exploring} - empirical evidence that maml also does rapid learning

% c finn s levine universality of gradient based meta-learning
% MAML has the same representational power as any other universal meta-learner
% depth is important for maml meta-learning

% frame it as MAML vs pre-training + FT

% http://www4.comp.polyu.edu.hk/~csxmwu/papers/NIPS-2020-Meta-Training.pdf
% compares support/query training vs leave-one-out training
% s/q generalization gap depends only on the number of meta-training tasks (assuming size of meta-training supprts equals size of meta-test support), while loo depends on both the number of tasks and the number of samples per task
% makes sense, this paper is not very significant imo
% also not clear whether the stability conditions hold

% ICLR workshop paper:
%EXPLORING THE SIMILARITY OF REPRESENTATIONS
% IN MODEL-AGNOSTIC META-LEARNING
% weights of early layers don't change very much even for pre-training, so it should not be used to conclude that MAML learns a rep, this is a universal property of neural nets
% 


% A recent line of work has shown that when a ground-truth representation of the data across tasks exists within the hypothesis class, then algorithms sharing similarities with MAML  can leverage all samples across tasks to learn it, which reduces  the sample complexity for a new task
%  . Further, experimental works have shown evidence that MAML learns an effective representation 
 
%  , suggesting that the virtue of algorithms for fast adaptation to new tasks, like MAML, is in effectively learning the low-dimensional representation. 
% \st{But neither MAML nor its variants have been provably shown to learn a more effective representation than classical algorithms, leaving the explanation for MAML's success yet to be found.} {\color{red} In this work, we instead focus on the 
% }



% {\color{red}but they do not consider iteration complexity

% While prior works study multi-task linear regression problems from a statistical perspective, viewing task sample complexity as the metric of algorithm success, we take a more optimization-based perspective. In our settings, the effective problem dimension is invariant across all tasks, so as a result the sample complexity is fixed.... In contrast, the


% ...still working...will finish asap in the morning
% }

% {\color{red}
% \cite{raghu2019rapid} posed two hypotheses to explain MAML's success in deep learning contexts. The first, known as {\em{feature reuse}}, claims that MAML learns a representation of the tasks' features, which enables high performance on new tasks sharing the representation, the second, known as {\em{rapid learning}}, posits that MAML finds a point in the optimization landscape well-suited for adaptation to new tasks via gradient descent. The authors empirically argued that MAML performs feature reuse, which was also supported by a series of subsequent works that showed sample-complexity improvements for MAML and other meta-learning algorithms when they learn a task representation in linear regression settings \citep{saunshi2020sample, tripuraneni2020provable, du2020fewshot}.

% there have been many works studying the representation leanring perspective, but our work focuses on the case when there may not be one.
% }
%These works assume that the tasks are linear regression problems belonging to some low-dimensional subspace, and show that meta-learning algorithms can implicitly learn this subspace \cite{saunshi2020sample}, or, explicitly solving for the subspace can reduce sample complexity. 
% Nevertheless, the jury is far from decided on an explanation for MAML's improvement relative to ERM: for instance, ERM is known to also perform feature reuse, and \cite{oh2020does} provided empirical evidence for the rapid learning hypothesis. In particular, this line of work leaves multiple related questions unanswered:
% \begin{itemize}
    % \item It is well understood that the tasks must obey some sort of structure in order for meta-learning to be useful. But must this shared structure be a low-dimensional representation? 
    %Standard meta-learning formulations only assume that the tasks are generated from the same distribution. Can we capture the advantage of the MAML solution over the ERM solution for broad classes of distributions, without assuming any shared low-dimensional representation among the tasks? 
    % \item Representation learning requires additional computation and parameters to learn and store the representation. Can we provably show that MAML achieves significant gain over ERM in settings with models lacking sufficient parameters to learn a representation?
%     \item Even when a low-dimensional representation may be learned, it has been shown in linear regression settings that ERM also finds this low-dimensional representation \citep{tripuraneni2020provable, du2020fewshot} at a fraction of the cost. In fact, the algorithms experimented with in \cite{raghu2019rapid, oh2020does} are versions of MAML that update only a fraction of the network parameters on each inner loop iteration, meaning that the other parameters are effectively trained via ERM. %Therefore, is MAML just re-purposed representation learning via ERM, or 
%     Thus, is there something unique about the MAML optimization landscape that yields a solution with unique, significant advantages over ERM?
% \end{itemize}

 \begin{figure*}[t]
% \vskip -0.1in
\begin{center}
%\centerline{\includegraphics[width=0.9\textwidth, height=3.9cm]{intro2.png}}
% for aistats 2 column, it was 0.21\textwidth
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/intro442.pdf}
         \includegraphics[width=\textwidth]{NeurIPS/intro4444.pdf}
         \caption{}
         \label{fig:y equals x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/intro112.pdf}
        \includegraphics[width=\textwidth]{NeurIPS/intro2222.pdf}
         \caption{}
         \label{fig:three sin x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/intro1111.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{NeurIPS/intro3333.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
     \vspace{-2mm}
        \caption{MAML, NAL excess risks and optimal solutions in various environments.}
        \label{fig:three graphs}
%\caption{Excess risks and optimal solutions for MAML and ERM in various types of task environments.}
 \vspace{-4mm}
\label{fig:eh_geo_gen}
\end{center}
% \vskip -0.1in
\end{figure*}
%  \vspace{-4mm}

% In this paper, we explain MAML's advantage over ERM in a multi-task linear regression setting.
% without assuming that MAML learns a more effective representation. 
% Indeed, we focus on computational complexity rather than sample complexity by defining task hardness in terms of the number of gradient descent steps required to reach the optimal solution.
%In this paper, 

% To do so, we obtain a general, optimization-based 
% perspective on the conditions required for MAML to improve over ERM in terms of few-shot regression performance.

% in a multi-task linear regression setting, 
% without assuming that MAML learns a more effective representation. 
% We focus on computational complexity rather than sample complexity by holding the effective problem dimension (and thus new task sample complexity) invariant across both algorithms, and 

% Recent works have shown that 

% In this work we focus on the latter

% While other works take a statistical perspective and equate task hardness with sample complexity \citep{saunshi2020sample, du2020few, tripuraneni2020provable}, we note that sample complexity depends on the effective problem dimension, and hence is invariant across tasks. 
% % Moreover, any algorithm that operate in the same effective dimension will have the same . 
% Complementary to this statistical perspective is the optimization perspective, which defines task hardness according to the landscape of the task's loss function. From the optimization perspective, hard tasks have losses with relatively flat curvatures, making them difficult for SGD to traverse quickly, whereas easy tasks have losses with steep curvatures, enabling SGD to quickly find the optimal solution. 
% %The strong convexity parameter of the task's loss function thus naturally parameterizes its hardness. 
% In our setting, loss function curvature and thus task hardness varies across tasks, allowing for a nuanced comparison between the types of solutions that MAML and ERM find within the global optimization landscape.

In particular, our main observations are best captured in the setting in which tasks are either ``hard" or ``easy". We let $\rho_H$ be the hardness parameter for the hard tasks, and $\rho_E$ be the hardness parameter for the easy tasks, where $\rho_E > \rho_H$ (smaller hardness parameter means more hard). As we measure the hardness of a task by the rate at which gradient descent converges for the task, in this case, the hardness parameter is the task loss function's strong convexity parameter. For a particular task environment, we let $R$ be the dimension-normalized distance between the average of easy tasks' optimal solutions and the average of hard tasks' optimal solutions, and let $r_H$ quantify the variance, or dispersion, of the hard tasks' optimal solutions. Assuming that $\frac{\rho_H}{\rho_E}(1-\frac{\rho_H}{\rho_E})^2 \gg \frac{d}{m}$, where $d$ is the problem dimension and $m$ is the number of samples used for adaptation,
%and the number of labeled samples $m$ available per task for gradient-based fine-tuning is order-wise at least 
% the $\Omega(d_{\text{eff}})$, where $d_{\text{eff}}$ is 
then
%if $d$ is the effective dimension of the problem, $\Omega(d)$
%two necessary and sufficient conditions for MAML to significantly improve upon ERM in this scenario:
% \vspace{-2mm}
% \begin{enumerate}
%     \item There must be significant difference between the difficulty of the easy and hard tasks.
%     \vspace{-2mm}
%     \item The optimal solutions of the hard tasks must be (a) close together and (b) far from the arithmetic center of the optimal solutions of the easy tasks. 
% \end{enumerate}
% \vspace{-2mm}
% To formalize these observations, we focus on a generic setting in which the task environment is a mixture of hard and easy tasks, where task hardness is inversely related to the strong convexity parameter of the task's loss function. Hard and easy tasks are drawn from the environment with equal probability, and the optimal solutions $\mathbf{w}_i^*\in  \mathbb{R}^d$ for hard tasks are sampled according to $\mathbf{w}_i^* \sim \mathcal{N}(R \mathbf{1}_d,r_H \mathbf{I}_d)$ and for easy tasks are sampled based on $\mathbf{w}_i^* \sim \mathcal{N}( \mathbf{0}_d,r_E \mathbf{I}_d)$.
%, and $D_{HH}$ measures the dispersion of the hard tasks. 
% Letting the strong convexity parameter of the easy tasks be $\rho_E = 1$, and that of the hard tasks be $\rho_H \in (0,0.5]$, 
%we find that for $m= \Omega(d)$, 
the ratio of the expected excess risks after task-specific adaptation of the NAL and MAML solutions is approximately (Corollary \ref{prop3}):
$\frac{\mathcal{E}_m(\mathbf{w}_{ERM})}{\mathcal{E}_m(\mathbf{w}_{MAML})} \approx 1 + \frac{ R^2}{r_{H}}$.
% \begin{align*}
%   %\frac{(1-\rho_H)^3 D_{HE}}{(1-\rho_H)^3 D_{HH} + O(\rho_H)} \leq \frac{f({w_{ERM}})}{f(w_{MAML})} \leq  \frac{(1-\rho_H)^3 D_{HE}+ O(\rho_H)}{(1-\rho_H)^3 D_{HH} }
% %   \quad \quad\quad \quad \quad \quad\quad 
% \frac{\mathcal{E}_m(\mathbf{w}_{ERM})}{\mathcal{E}_m(\mathbf{w}_{MAML})} \approx 1 + \frac{ R^2}{r_{H}} .
% \end{align*} 
% ratio for general $\rho_E$:
% $ \frac{\rho_E^2 r_H + \rho_E R^2}{\rho_H()}$
Thus, 
the largest gain for MAML over NAL occurs when the task environment satisfies (informal): 
% (I) the hard tasks are significantly more difficult than the easy tasks $\frac{\rho_H}{\rho_E}\ll 1$, without being impossibly hard ($\rho_H \geq c > 0$), and
%     (II) {\em Benign geography:} the optimal solutions of the hard tasks have small variance $r_H$, and the distance between the hard and easy task centers $R$ is large.
  \vspace{-2mm}
 \renewcommand{\theenumi}{\Roman{enumi}}
 \begin{enumerate}
  \item {\em Hardness discrepancy:} the hard tasks are significantly more difficult than the easy tasks $\frac{\rho_H}{\rho_E}\ll 1$, without being impossibly hard ($\rho_H \geq c > 0$), and
  \vspace{-1mm}
    \item {\em Benign geography:} the optimal solutions of the hard tasks have small variance $r_H$, and the distance between the hard and easy task centers $R$ is large.
      \vspace{-2mm}
 \end{enumerate}
 Figure \ref{fig:eh_geo_gen} summarizes observations (I) and (II) by plotting locations of the easy and hard tasks' optimal solutions sampled from four distinct task environments and the corresponding solutions and excess risks for NAL and MAML. The environment in subfigure (a) violates (I) since $\frac{\rho_H}{\rho_E}=1$. Subfigures (b)-(c) show environments with either small $R$ or  large $r_h$, so  (II) is not satisfied. In contrast, the environment in subfigure (d) has small $r_H$, large $R$, and $\frac{\rho_H}{\rho_E}\!=\!0.2$, in which case as expected MAML achieves the largest gain over NAL, $\frac{\mathcal{E}_m(\mathbf{w}_{NAL})}{\mathcal{E}_m(\mathbf{w}_{MAML})} \approx 3 $.

\textbf{Summary -- Why MAML.} We show  theoretically and empirically that MAML outperforms standard training (NAL) in linear and nonlinear settings by finding a solution that excels on the more-difficult-to-optimize (hard) tasks, as long as the hard tasks are sufficiently similar. Our work thus highlights the importance of task hardness and task geography to the success of MAML.
% giving practitioners valuable insights on when to use it.

% Our results theoretically justify the empirical benefits of focusing on the hard tasks while training meta-learning methods \cite{zhou2020expert,sun2020meta} 
% and provide intuition to practitioners on when they can save computational resources by  using standard ERM for meta-learning instead of the more expensive MAML. 


 
% We formalize these observations in Sections 3 and 4. Next, we argue that these observations generalize beyond mixed linear regression to mixed regression with two-layer neural networks with smooth activations in Section 5. Finally we show that these insights further generalize to few-shot image classification settings  in Section 6.
 
% We note that this result requires $m$ to be $m=\Omega(d_{\text{eff}})$, and the motivation for MAML is to find a model that can adapt to new tasks with very little training data, i.e., small $m$. However, we conjecture that in deep learning in which MAML is typically used, $d_{\text{eff}}$ is typically small because both MAML and ERM reduce the problem to low dimensions by learning a representation of the tasks. To support this, we study the case in which the learning model is a two-layer linear neural network, and show that 
% given an accurate representation in the first layer, the effective dimension of the problem is indeed reduced.

% {\color{red} learning an accurate representation in the first layer} indeed reduces the effective dimension of the problem. 
% In the following sections we explain this result, starting with a summary of notations and a more formal exposition of the problem setting.

% \begin{figure}[t]
% \vskip -0.1in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{geo_intro2.png}}
% \caption{Examples of locations of easy and hard task optimal solutions for various $D_{HE}$ and $D_{HH}$.}
% \label{fig:geo_intro}
% \end{center}
% \vskip -0.4in
% \end{figure}



%We also consider the case where we do indeed have access to a multilayer regressor, in particular a two-layer linear neural network, and analyze when MAML performs significantly better than ERM, under the assumption of a low-dimensional generative model for the task-optimal solutions.

%doing so not only relies on the assumption of an existing low-dimensional structure, but also requires additional parameters to be added to the regressor, thereby making the problem nonconvex. 
%It is well understood that the tasks must obey some sort of structure in order for meta-learning to be useful. In its most general form, this structure manifests in the typical meta-learning assumption that the tasks are all drawn from the same distribution, referred to as the task environment. When analyzing meta-learning for linear regression, prior works have
%Our particular contributions can be summarized as follows:
%\begin{itemize}
%    \item We show that MAML provides performance gains over ERM even in the simplest two-task, convex linear regression setting when there is appropriate discrepancy in the hardness, i.e. condition number, of the tasks. 
%    \item In the multi-task case with all tasks being either easy or hard, we show that MAML significantly outperforms ERM only when two geometric conditions of the task optimal solutions are satisfied, again without assuming any low-dimensional representation nor a multi-layer regressor. 
    %\item {\color{red}In the case that the regressor is a two-layer neural network and there exists a low-dimensional representation of the tasks, we show that both MAML and ERM find it? We show similar conditions on the tasks for when MAML significantly outperforms ERM}
    %\item {\color{red}We show experimentally that these insights hold for image classification experiments with a multi-layer neural network. In particular, ... use MNIST for easy tasks, F-MNIST for hard tasks? probably not hard enough. FEMNIST? maybe should focus on federated settings, unless we explicitly consider a task environment with new meta-test tasks. For deep learning experiments incorporating hardness, compare to this paper https://arxiv.org/pdf/2007.06240v1.pdf}
%\end{itemize}

\input{NeurIPS/Related_Work}

%\subsection{Notation} We use boldface uppercase for matrices and boldface lowercase for vectors. For a vector $\mathbf{u}$, we denote 
% their inner product by $\langle \mathbf{u}, \mathbf{v} \rangle = \mathbf{u}^\top \mathbf{v}$, the norm induced by the matrix $\mathbf{A}$ as $\|\mathbf{u}\|_\mathbf{A}^2 \coloneqq {\mathbf{u}^\top \mathbf{A} \mathbf{u}}$. We use $\|\mathbf{A}\|_2$ to denote the spectral norm of $\mathbf{A}$. We denote the $d\times d$ identity matrix by $\mathbf{I}_d $ and the $d$-dimensional vector of zeros (ones) by $\mathbf{0}_d$ ($\mathbf{1}_d$). We represent the multivariate Gaussian distribution with mean $\mathbf{0}_d$ and covariance $\mathbf{\Sigma}$ by $\mathcal{N}(\mathbf{0}, \mathbf{\Sigma})$.

% to do:

%reorg- section 3.2 up front, everything else explains it
% remove equations, make things inline
% plots of task locations
% section at end with more numerical results
% include numerical results in early version of section 3.2? or just include plots of the equations, tbd
% on other paper: just write down the rates for the 3 algs, currently what i have is a mix. also read constantine's paper

% to do: 
% condense special case corollary section
% come up with plan for experiments

% to do:
% rhoH/rhoE in intro
% plots
% experiment section
% related work




==> NeurIPS/Multitask.tex <==
%!TEX root = main.tex
\section{Multi-Task Linear Regression}
\label{section:linear}
We first explore the relative behaviors of MAML and NAL in a setting in which we can obtain closed-form solutions: multi-task linear regression. Here, the model $h_\mathbf{w}$ maps inputs $\mathbf{x}$ to predicted labels by taking the inner product with $\mathbf{w}$, i.e. $h_\mathbf{w}(\mathbf{x})\! =\! \langle\mathbf{w}, \mathbf{x}\rangle$. The loss function $\ell$ is the squared loss, therefore $f_i(\mathbf{w})\! =\! \frac{1}{2}\mathbb{E}_{(\mathbf{x}_i, {y}_i)\sim \mu_i}[(\langle\mathbf{w}, \mathbf{x}\rangle\! -\! y_i)^2]$ and $\hat{f}_i(\mathbf{w}; \mathbf{X}_i, \mathbf{y}_i)\!=\! \frac{1}{2}\|\mathbf{X}_i\mathbf{w}\! -\! \mathbf{y}_i\|_2^2$  for all $i$.
We consider a realizable setting in which the data for the $i$-th task is Gaussian and generated by a ground truth model $\mathbf{w}_{i,\ast}\! \in\! \mathbb{R}^d$. That is, points $(\mathbf{x}_i,y_i)$ are sampled from $\mu_i$ by first sampling $\mathbf{x}_i\! \sim\! \mathcal{N}(\mathbf{0}, \mathbf{\Sigma}_i)$, then sampling $y_i \sim \mathcal{N}(\langle \mathbf{w}_{i,\ast}, \mathbf{x}_i \rangle, \nu^2 )$, i.e. $y_i\! =\! \langle \mathbf{w}_{i,\ast}, \mathbf{x}_i \rangle\! +\! z_i$ where $z_i\! \sim\! \mathcal{N}(0, \nu^2)$.
%we don't need to add any more equations, other than maybe state the excess risk
% In this setting the excess risk is given by 
% \begin{align} \label{eq:excess_risk}
%     \mathcal{E}_m(\mathbf{w}) &= F_m(\mathbf{w}) - \tfrac{1}{2} \mathbb{E}_{i}\big[ \sigma^2 + \tfrac{\alpha^2 \sigma^2}{m} \text{tr} ( \mathbf{\Sigma}_i^2)\big] =  \tfrac{1}{2}  \mathbb{E}_{\mathcal{T}_i,\mathbf{\hat{X}}_i}\big \| \mathbf{\tilde{P}}_i(\mathbf{w} - \mathbf{w}_i^\ast) \|^2_{\mathbf{\Sigma}_i}\big],
% \end{align}
% where $\mathbf{\hat{P}}_i \coloneqq \mathbf{I}_d -  \tfrac{\alpha}{m}\mathbf{\hat{X}}_i^\top \mathbf{\hat{X}}_i$ for all $i$. 
In this setting the population-optimal solutions for NAL and MAML 
%(the minimizers of (\ref{}) ) 
are given by:
\begin{align}
    \mathbf{w}_{NAL}^\ast &= \mathbb{E}_{i}[\mathbf{\Sigma}_i]^{-1} \mathbb{E}_{i}[\mathbf{\Sigma}_i \mathbf{w}_i^\ast], \quad \text{ and } \quad % \label{erm_pop} 
    \mathbf{w}_{MAML}^\ast = \mathbb{E}_{i}[\mathbf{Q}_i^{(n_2)}]^{-1} \mathbb{E}_{i}[\mathbf{Q}_i^{(n_2)} \mathbf{w}_i^\ast], \label{maml_pop}
\end{align}
where for any $s\in \mathbb{N}$, we define
% \vspace{-3mm}
% \begin{equation} \label{Q}
    $\mathbf{Q}_i^{(s)}\! \coloneqq ( \mathbf{I}_d\!-\! \alpha \mathbf{\Sigma}_i )\mathbf{\Sigma}_i ( \mathbf{I}_d\!-\!\alpha \mathbf{\Sigma}_i ) +  \frac{\alpha^2}{s}(\text{tr}(\mathbf{\Sigma}_i^2) \mathbf{\Sigma}_i \!+\! \mathbf{\Sigma}_i^3)$.
    % \vspace{-3mm}
% \end{equation}
% These $\mathbf{Q}_i^{(s)}$ matrices arise due to the stochastic gradient step in the MAML objective and play the role of the covariance matrices $\mathbf{\Sigma}_i$ in the NAL solution. They are composed of two terms: a preconditioned covariance matrix $\mathbf{\Sigma}_i \left( \mathbf{I}_d- \alpha \mathbf{\Sigma}_i \right)^2$, and a perturbation matrix due to the stochastic gradient variance.% Assuming that the sum of the empirical covariance matrices for each task is invertible, 
% We focus on comparing the  behavior of these population-optimal solutions in the majority of the analysis in this section. 
Note that these $\mathbf{Q}_i^{(s)}$ matrices  are composed of two terms: a preconditioned covariance matrix $\mathbf{\Sigma}_i \left( \mathbf{I}_d- \alpha \mathbf{\Sigma}_i \right)^2$, and a perturbation matrix due to the stochastic gradient variance.
We provide expressions for the empirical solutions $\mathbf{w}_{NAL}$ and $\mathbf{w}_{MAML}$ for this setting and show that they converge to $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ as $n,T,\tau \rightarrow \infty$ in Appendix \ref{app:converge}. Since our focus is ultimately on the nature of the solutions sought by MAML and NAL, not on their non-asymptotic behavior, we analyze  $\mathbf{w}_{NAL}^\ast$ and $\mathbf{w}_{MAML}^\ast$ in the remainder of this section, starting with the following result.

% can we modify our NAL result to capture the dependence on the variance of the matrices?
% can we 

%$\mathbf{Q}_i^{(a)} = \mathbf{\Sigma}_i \left( \mathbf{I}_d- \alpha \mathbf{\Sigma}_i \right)^2 +  \frac{\alpha^2}{a}(\text{tr}(\mathbf{\Sigma}_i^2) \mathbf{\Sigma}_i + \mathbf{\Sigma}_i^3)$

% While NAL converges with $T$ and $n$, MAML converges with $T$ and $\tau$, since it trains on task episodes instead of individual samples. {\color{red} The convergence rate for NAL is faster due to the fact that the eigenvalues of $\mathbf{Q}_i$ are smaller than the eigenvalues of $\mathbf{\Sigma}_i$.}
% % as the slowest diminishing term is $\mathcal{O}(\exp\left(-b\right))$ for NAL and  $\mathcal{O}(\exp\left(-b^{1/3})\right)$ for MAML. 
% This provides more evidence that the MAML solution is more difficult to compute than the NAL solution, highlighting the need to understand by how much the MAML solution improves on the NAL solution in certain scenarios. 
%We characterize the excess risks of the NAL and MAML population-optimal solutions in the next result.

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{2tasks_inffin_msmall_theory.png}}
% \caption{Theoretical losses for the setting described directly above.
% }
% \label{fig_finfin_n1n2_10_thr}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{2tasks_largem.png}}
% \caption{\textbf{Fixed large $m$, varying $n_2$.} Experimental losses for GD and MAML when given $(n_1,n_2) = (1000,n_2)$ meta-training samples on each meta-training iterations, and $m=1000$ samples at meta-test time. Each subplot shows the total loss over varying $r_{k^\ast}$, with $\sigma_{1,1}^2$, $\sigma_{2,1}^2$, and $\sigma_{2,2}^2$ held constant at 1. %Note that GD has access to $n_1 + n_2 = n$ samples during meta-testing, so for this experiment it always has access to at least 1000 meta-training samples.
% }
% \label{fig_finfin_n2}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure}[H]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{inf_fin_mfixed.png}}
% \caption{Theoretical results for setting described above.}
% \label{mfixed_theory}
% \end{center}
% \vskip -0.2in
% \end{figure}

%To further understand these excess risk functions, we next analyze them through a simple example.


%We can also show that the excess risks converge to each other when $m$ is small, which we show in the Appendix.
% Using this result, we can imagine a realistic setting in which MAML achieves quantifiable gain over NAL. Suppose tasks are drawn from a mixture distribution of hard and easy tasks. First the hard or easy task type is selected, each with probability 1/2. If the task type is hard, then the optimal solution is selected from a Euclidean ball of radius $R$ and center that is a distance $M$ from the origin. If the easy task type is selected, then the task optimal solution is drawn from the Gaussian measure over $\mathbb{R}^d$ with mean 0 and variance $\nu^2$. In this scenario, we have
% \begin{align}
%     D_{HH} &\leq \tfrac{T}{2}(R T)^2 = \tfrac{1}{2} T^3 R^2
% \end{align}
% and with high probability $h(\delta)$,
% \begin{align}
%     D_{HE} &\geq \tfrac{T}{2}(\tfrac{T}{2}T(M-R-\delta))^2 = \tfrac{1}{8}T^3 (M-R-\delta)^2
% \end{align}
% because each hard task is a distance at least $M-R$ from the origin, which yields an average displacement of $M-R$ from a randomly drawn easy task, times the number of easy tasks gives the result. 
% Then we have
% \begin{align}
% \frac{f(\mathbf{w}_{NAL}^\ast)}{f(\mathbf{w}_{MAML}^\ast)}
%     &\geq \frac{ (1- \rho_H)^3D_{HE} }{(1-\rho_H)^3 D_{HH} + \mathcal{O}(\rho_H)} \nonumber \\
%     &\geq \frac{ (1- \rho_H)^3 T^3 (M-R-\delta)^2 }{4(1-\rho_H)^3 T^3 R^2 + \mathcal{O}(\rho_H)} \\
%     &\approx\frac{ (M-R-\delta)^2 }{4R^2}
% \end{align}
% Next, suppose that the center of the hard tasks is also drawn from the Gaussian measure over $\mathbb{R}^d$ with mean 0 and variance $\nu^2$. Then by concentration of measure theory, $M \in [\nu\sqrt{d}-\epsilon, \nu\sqrt{d}+\epsilon]$ with exponentially high probability. This yields
% \begin{align}
% \frac{f(\mathbf{w}_{NAL}^\ast)}{f(\mathbf{w}_{MAML}^\ast)}
%     &\geq \frac{ (\nu\sqrt{d}-R-\epsilon-\delta)^2 }{4R^2} \\
%     &\approx \frac{\nu^2 d}{4R^2} - \frac{\nu \sqrt{d}}{2R}  %+ \frac{1}{4}
% \end{align}
% with exponentially large probability.


==> NeurIPS/Nonlinear.tex <==
\vspace{-0mm}
\section{Two-layer Neural Network}
\vspace{0mm}
\label{section:nonlinear}
% {\color{red} Choose one of the two results below to keep}


% Next, we use this result to show that MAML prioritizes performance on the hard task in the special case in which the learning model is a single neuron.

In this section, we consider a  non-linear setting in which each task is a regression problem with a two-layer neural network with a fixed second layer. The $k$-th neuron in the network maps $\mathbb{R}^d \rightarrow \mathbb{R}$ via $\sigma(\langle \mathbf{w}^k, \mathbf{x}\rangle )$, where $\sigma : \mathbb{R} \rightarrow \mathbb{R}$ is some activation function and $\mathbf{w}^k \!\in\!\mathbb{R}^d$ is the parameter vector. The network contains $M$ neurons for a total of $D =Md$ parameters, which are contained in the matrix $\mathbf{W} \coloneqq [\mathbf{w}^1, \dots, \mathbf{w}^M] \in \mathbb{R}^{d \times M}$. The predicted label for the data point $\mathbf{x}$ is the sum of the neuron outputs, namely $h_\mathbf{W}(\mathbf{x}) \coloneqq \sum_{k=1}^M \sigma(\langle\mathbf{w}^k, \mathbf{x}\rangle)$. The loss function is again the squared loss, i.e. $f_i(\mathbf{W}) = \frac{1}{2}\mathbb{E}_{(\mathbf{x}_i, {y}_i)\sim \mu_i}[(\sigma(\sum_{k=1}^M\langle\mathbf{w}^k, \mathbf{x}_i\rangle) - y_i)^2]$. Ground-truth models $\mathbf{W}_{i,\ast}$ generate the data for task $i$. We sample $(\mathbf{x}_i, y_i) \sim \mu_i$ by first sampling $\mathbf{x}_i \sim \mathcal{N}(\mathbf{0}_d, \mathbf{\Sigma}_i)$ then computing $y_i = \sum_{k=1}^M \sigma(\langle \mathbf{w}_{i,\ast}^k, \mathbf{x}_i\rangle)$. 
The following result demonstrates an important property of the MAML objective function in the two-task version of this setting.

% We first cite a result adapted from \cite{zhong2017recovery} which shows that $f_i$ is strongly convex and smooth close to the ground-truth. The result holds for a broad class of activations formally described in \cite{zhong2017recovery} that includes ReLU, Softplus and any nonlinear non-decreasing smooth function with bounded symmetric derivative, e.g. Sigmoid and tanh.


% We prove that in this setting, when there is sufficient difference in hardness among the tasks, MAML initializes closer to the hard task. 

% need to: 1. justify notion of hardness. 2. compute hessian.
% Gradient:
% \mathbf{w} is vectorized \mathbf{W}.

% Prior work has shown that under mild regularity assumptions, the hardness of learning a neuron (the number of gradient steps required) is again related to the covariance of the data distribution (see Theorems 3.2 and 4.2 in \citep{yehudai2020learning}). Thus we set $\mathbf{\Sigma}_i = \rho_H \mathbf{I}_d$ and $\mathbf{\Sigma}_{i'} = \rho_E \mathbf{I}_d$ for hard and easy tasks, respectively, with $\rho_H < \rho_E$.



% \citet{zhong2017recovery} shown that the Hessian for two-layer neural networks with a broad class of activations is locally positive definite around the global optimal solution. 

% need to state our new result showing that minimum eigenval scales with data variance.

% We require to $\sigma$ to satisfy multiple properties which we defer to the appendix for now

\begin{theorem}\label{lem:sc}
% [Application of Lemmas D.3, D.10 from \cite{zhong2017recovery}] 
% Assume that $\sigma$ satisfies Properties 3.1-3.3 from \cite{zhong2017recovery}.
%, in particular, that $\sigma$ is $\gamma$-homogeneous (see Appendix ).
Suppose that in the setting described above, the task environment is the uniform distribution over two tasks, and $\sigma$ is the ReLU, Softplus, Sigmoid, or tanh function.
Let $\mathbf{\Sigma}_i \!=\! \mathbf{I}_d$ and define $s_{i,k}$ as the $k$-th singular value of $\mathbf{W}_{i,\ast}$, $\kappa_i \coloneqq \|\mathbf{W}_{i,\ast}\|_2/s_{i,M}$, and $\lambda_i \coloneqq \frac{\Pi_{k=1}^M s_{i,k}}{s_{i,M}^M}$ for $i\!\in\!\{1,2\}$.
Further, define the regions
% Then the population loss $f_i$ is strongly convex and smooth in the region 
$\mathcal{S}_i \coloneqq \{\mathbf{W} : \|\mathbf{W} - \mathbf{W}_{i,\ast}\|_2 \leq c_1 /(s_{i,1}^c \lambda_i \kappa_i^2 M^2)\}$
and the parameters $\beta_i \coloneqq \frac{c_2}{\lambda_i \kappa_i^2}$ and $L_i \coloneqq c_3 M s_{i,1}^{2c}$ for $i \in \{1,2\}$ and absolute constants $c,c_1,c_2,$ and $c_3$. Let $\beta_1\!<\!\beta_2$ and $L_1\!<\!L_2$.
% define alpha, 
For   any stationary point $\mathbf{W}_{MAML}^\ast$ of the population MAML objective (\ref{exp_test}) with full inner gradient step ($m=\infty$), such that $\mathbf{W}_{MAML}^\ast\!\in \mathcal{S}_1 \cap \mathcal{S}_2$, must satisfy for all $\alpha \leq 1/L_2$:
%$\! \in \mathcal{S}_1 \cap \mathcal{S}_2$ is a stationary point of 
% with parameters $\beta_i \coloneqq \frac{c_2}{\lambda_i \kappa_i^2}$ and $L_i \coloneqq c_3 M s_{i,1}^{2c}$, respectively, where $c,c_1,c_2$ and $c_3$ are absolute constants, for $i$.
% \begin{align}
% \beta_i &\coloneqq \frac{c }{\lambda \kappa^2} - c' M^2 \sigma_{i,1}^\gamma \|\mathbf{W} - \mathbf{W}_{i,\ast}\|_2 \nonumber \\
% L_i &\coloneqq c M \| \mathbf{W}_{i,\ast}\|_2^{2p} + c' M^2 \| \mathbf{W}_{i,\ast}\|_2^\gamma \|\mathbf{W} - \mathbf{W}_{i,\ast}\|_2
% \end{align}
% Suppose that the task environment $p$ contains two tasks, with task 1 being the hard task and task 2 the easy task. 
% Let $\mathcal{S}_1, \mathcal{S}_2, \beta_1,L_1, \beta_2, $ and $L_2$ be as defined in Proposition \ref{lem:sc}. 
% Since task 1 is hard, we have $\beta_2 > \beta_1$, and we further assume $L_2 > L_1$.  Let the step size $\alpha = 1/L_2$. Then
%$\mathbf{W}_1 \coloneqq \mathbf{W}_{MAML} - \alpha \nabla f_1(\mathbf{W}_{MAML})$ and $\mathbf{W}_2 \coloneqq \mathbf{W}_{MAML} - \alpha \nabla f_2(\mathbf{W}_{MAML})$,  where $\alpha = 1/L_2$. Then 
\begin{equation}
    \| \nabla f_1(\mathbf{W}_{MAML}) \|_2 \leq {\frac{1 - 2\alpha\beta_2}{(1- \alpha L_1)^2}} \|\nabla f_2(\mathbf{W}_{MAML})\|_2 + O(\alpha^2).
\end{equation}
\vspace{-2mm}
% 0.0003
% \begin{align}
%     \lambda_{\max}(\nabla^2 f_i(
%     \mathbf{W})) \leq  c M \| \mathbf{W}_{i,\ast}\|_2^{2p} + c' M^2 \| \mathbf{W}_{i,\ast}\|_2^p \|\mathbf{W} - \mathbf{W}_{i,\ast}\|_2
% \end{align}
% is the scaling actually rho
% what to set the difference to be -- include rho here. but the smaller that rho is, the closer the init needs to be to the GT, so itcircular
% lemma D.10:
% $\|\nabla^2 f_i(\mathbf{W}) - \nabla^2 f_i(\mathbf{W}_{i,\ast})\| \leq c M^2 \| \mathbf{W}_{i,\ast}\|_2^p \|\mathbf{W} - \mathbf{W}_{i,\ast}\|_2$. % p is degree of homogeneity of activation? can we get rid of the M dependence by using avg instead of sum? combine these results
\end{theorem}
\textbf{Interpretation: MAML prioritizes hard tasks.} In the setting above, {$\beta_i$ and $L_i$ are strong convexity and smoothness parameters, respectively, of the function $f_i$ on the region $\mathcal{S}_i$.
% described in Theorem \ref{lem:sc}, 
Here,} task 1 is the harder task since $\beta_1$ and $\beta_2$ control the rate with which gradient descent converges to the ground-truth solutions \citep{zhong2017recovery}, with smaller $\beta_i$ implying slower convergence, and $\beta_1 < \beta_2$. Thus, Theorem
\ref{lem:sc}
shows that, any stationary point of the MAML objective in $\mathcal{S}_1 \cap \mathcal{S}_2$ has smaller gradient norm on the hard task than on the easy task as long as there is sufficient hardness discrepancy, specifically $\beta_2 > L_1$. {Physically, this
condition means that the curvature of the loss function for the easy task is more steep than the curvature of the hard task in all directions around their ground-truth solutions.}
The smaller gradient norm of MAML stationary points on the harder task suggests that {\em  MAML solutions prioritize hard-task performance.} 
% Note that the conditioning of the ground-truth solution $\mathbf{W}_{i,\ast}$ determines the hardness of task $i$ in this setting. % how to explain that inverse condition number is strong convexity parameter....
% Since the losses $f_1$ and $f_2$ are strongly convex in this region, this implies that the MAML solution is closer to the optimal solution of the hard task. 
In contrast, we can easily see that any stationary point $\mathbf{w}_{NAL}$ of the NAL population loss must satisfy the condition $\|\nabla f_1 (\mathbf{w}_{NAL})\|_2 = \|\nabla f_2 (\mathbf{w}_{NAL})\|_2$, meaning that {\em NAL has no such preference for the hard task.}


% then this stationary point must be such that the gradient of the hard task loss after adaptation has smaller norm than that of the easy task as long as there is sufficient hardness discrepancy, specifically $\beta_2 > L_1$. Since $f_1$ and $f_2$ are locally strongly convex and smooth, the smaller gradient of the hard task suggests that MAML performs better after one step of adaptation on the hard task than the easy task. 

% Using this result, we show that in a two-task setting, if a stationary point of the MAML objective exists in $\mathcal{S}_1 \cap \mathcal{S}_2$, then this point has smaller on the hard task after updating as it does on the easy task.


% \textbf{Visualizations.}  Figures \ref{fig:softplus}  and \ref{fig:sigmoid} 
% demonstrate the importance of task hardness and geography in comparing NAL and MAML in this setting. Here, for ease of visualization we consider the case in which $M=1$ and $d=2$, i.e. the learning model consists of one neuron mapping from $\mathbb{R}^2 \rightarrow \mathbb{R}$. Each subfigure plots the NAL or MAML loss landscape for different task environments with different activations $\sigma$, as well as the ground-truth neuron for each task. Figure \ref{fig:softplus} uses the Softplus function while Figure \ref{fig:sigmoid}  uses the Sigmoid function.  In light of prior work showing that the number of gradient steps required to learn a single neuron diminishes with the variance of the data distribution (Theorem 3.2 in \cite{yehudai2020learning}), we again control task hardness by varying the data variance. In  all plots, $\mathbf{\Sigma}_i = 0.5 \mathbf{I}_2$ for hard tasks and $\mathbf{\Sigma}_i =  \mathbf{I}_2$ for easy tasks. Lastly, we would like to note that the MAML loss is the true evaluation metric, as we are ultimately concerned with model performance after one step of task-specific adaptation. 

% Figure \ref{fig:softplus}  shows that when all tasks are equally hard, the MAML and NAL solutions are similar (a-b), whereas when one task is hard, MAML initializes closer to the hard task and achieves significantly better post-adaptation performance than the NAL solution (c-d). 
% In the same vein, Figure \ref{fig:sigmoid}  demonstrates that when the tasks are uniformly dispersed (large $r_H$, small $R$), the NAL and MAML solutions are similar, whereas when the hard tasks are clustered away from the center of the easy tasks (small $r_H$, large $R$), MAML initializes closer to the hard tasks and substantially outperforms NAL (c-d). 

% ----------

% Figure \ref{fig:softplus}
% demonstrates the importance of task hardness in comparing NAL and MAML in this setting. Here, for ease of visualization we consider the case in which $M=1$ and $d=2$, i.e. the learning model consists of one neuron (with Softplus activation) mapping from $\mathbb{R}^2 \rightarrow \mathbb{R}$. Each subfigure plots the NAL or MAML loss landscape for different task environments, as well as the ground-truth neuron for each task. % Figure \ref{fig:softplus} uses the Softplus function while Figure \ref{fig:sigmoid}  uses the Sigmoid function.  
% In light of prior work showing that the number of gradient steps required to learn a single neuron diminishes with the variance of the data distribution (Theorem 3.2 in \cite{yehudai2020learning}), we again control task hardness by varying the data variance. In  all plots, $\mathbf{\Sigma}_i = 0.5 \mathbf{I}_2$ for hard tasks and $\mathbf{\Sigma}_i =  \mathbf{I}_2$ for easy tasks. Lastly, we would like to note that the MAML loss is the true evaluation metric, as we are ultimately concerned with model performance after one step of task-specific adaptation. 

% We observe that when all tasks are equally hard, the MAML and NAL solutions are similar (subfigures (a)-(b)), whereas when one task is hard, MAML initializes closer to the hard task and achieves significantly better post-adaptation performance than the NAL solution (c)-(d), supporting our intuition that MAML achieves significant gain over NAL in task environments in which it can leverage improved performance on hard tasks. 
%------

Figure \ref{fig:softplus}
demonstrates the importance of task hardness in comparing NAL and MAML in this setting. Here, for ease of visualization we consider the case in which $M=1$ and $d=2$, i.e. the learning model consists of one neuron (with Softplus activation) mapping from $\mathbb{R}^2 \rightarrow \mathbb{R}$. Each subfigure plots the NAL or MAML population loss landscape for different task environments with $m\!=\!250$, as well as the ground-truth neuron for each task. % Figure \ref{fig:softplus} uses the Softplus function while Figure \ref{fig:sigmoid}  uses the Sigmoid function.  
In light of prior work showing that the number of gradient steps required to learn a single neuron diminishes with the variance of the data distribution (Theorem 3.2 in \cite{yehudai2020learning}), we again control task hardness via the data variance. In all plots, $\mathbf{\Sigma}_i = 0.5 \mathbf{I}_2$ for hard tasks and $\mathbf{\Sigma}_i =  \mathbf{I}_2$ for easy tasks. Note that the MAML loss (evaluated after one step of adaptation) is the evaluation metric we ultimately care about. 

We observe that when all tasks are equally hard, the MAML and NAL solutions are identical (subfigures (a)-(b)), whereas when one task is hard, MAML initializes closer to the hard task and achieves significantly better post-adaptation performance than the NAL solution, which is closer to the centroid of the easy tasks (c)-(d). This supports our intuition that MAML achieves significant gain over NAL in task environments in which it can leverage improved performance on hard tasks. 

% \textbf{Limitations.} For simplicity we only theoretically consider a setting with two tasks and analyze stationary points close to the ground-truth models. However, based on our analysis generalizing the two-task linear case to many tasks (Sections \ref{section:hardness} and \ref{section:linear_experiments}), as well as our numerical simulations (Figure \ref{fig:softplus}), we believe that MAML also prioritizes performance on hard tasks in many-task non-linear settings. 
% Additionally, we conjecture that our insights also apply for globally non-convex landscapes in the sense that MAML finds a solution closer to local minima of hard tasks than those of easy tasks. 
% We conjecture352that our insights apply to general nonconvex landscapes under an expanded notion of closeness of353solutions: namely, that MAML prioritizesperformanceon the hard tasks by initializing close to a354local minima, rather than initializing close to the global optimum, but we do not analyze this
% In the same vein, Figure \ref{fig:sigmoid}  demonstrates that when the tasks are uniformly dispersed (large $r_H$, small $R$), the NAL and MAML solutions are similar, whereas when the hard tasks are clustered away from the center of the easy tasks (small $r_H$, large $R$), MAML initializes closer to the hard tasks and substantially outperforms NAL (c-d). 



% The following quantitative result aims to help explain this behavior.

% \cite{yehudai2020learning} 

% We begin by first showing that the task hardness task is again related to data covariance.
% Figure \ref{fig:} shows the effect of task hardness 

% that MAML initializes closer to the hard task than NAL does, 

% \begin{proposition}\label{prop:sc}
% Suppose $\sigma(\cdot)$ is the Softplus activation, i.e. $\sigma(z) = \log(1+e^z)$. 
% % Then $f_1$ and $f_2$ are strongly convex with parameters $\rho_H$ and $\rho_E$, respectively.
% Let $\mathbf{w}_{MAML}$ be a stationary point of the MAML objective, and let $\mathbf{w}_1 = \mathbf{w}_{MAML} - \alpha \nabla f_1(\mathbf{w}_{MAML})$ and $\mathbf{w}_2 = \mathbf{w}_{MAML} - \alpha \nabla f_2(\mathbf{w}_{MAML})$ for some sufficiently small $\alpha$. 
% % Assume that $ c(\rho_H) \geq \|\mathbf{w}_{MAML} - \mathbf{w}_{1,\ast}\|_2$ and $ c(\rho_E) \geq \|\mathbf{w}_{MAML} - \mathbf{w}_{2,\ast}\|_2$.
% If $4\rho_H< \rho_E$, then $\|\mathbf{g}_1(\mathbf{w}_1)\|_2 < \|\mathbf{g}_2(\mathbf{w}_2)\|_2$.
% \end{proposition}

% The above result involves showing that the loss function for the Softplus activation is strongly convex under the specified conditions, then applying a general result for strongly convex functions given in the Appendix. The smaller gradient norm for task 1 implies that MAML prioritizes performance on the harder task, as we observed 
% % and helps to explain MAML's tendency to initialize closer to the task with larger data variance 
% in Figure \ref{fig:softplus}. 

% This result cannot be extended to the case of sigmoid activation because sigmoid yields a non-convex loss. However, Figure \ref{fig:sigmoid} suggests that our conclusions about the importance of $r_{H}$ and $R$ generalize even to nonconvex settings, which we further explore in the next section. 



%what is c1, c2?

% \begin{proposition}[Hardness] \label{prop:nonlinear}
% In the setting described above, any stationary point of the MAML objective satisfies that 
% % \begin{align}
% % \end{align}
% % say that MAML does better on the hard task than NAL
% % steps:
% % justify appropriate choice of alpha
% % appropriate choice of alpha --> grad closer to 0
% % grad closer to 0 --> similar performance (loss closer to 0)
% % compare to NAL
% % gemeralize?
% \end{proposition}

% We again consider a two-task environment with $\mathbf{\Sigma}_1 = \rho_E \mathbf{I}_d$ and $\mathbf{\Sigma}_2 = \rho_H \mathbf{I}_d$. Here the

% $n=500, T=4, \tau = 5, n_1 = 20, n_2= 80$

% \subsection{Task Hardness and Geography}



% we can show that hardness is related to the data variance, see learning a single neuron paper.
% can we show that maml picks the harder task?
% need to use the fact that maml incorporates minimum eigenval of hessian somehow...
% if resolvent is larger, we need grad of loss to be smaller... 
% must be proportional to that of other task.step size is 1/max(Sigma1, Sigma2) so the easier task has zero grad error. the harder task then must have grad after update equal to zero. we need 


% For MAML, $w$ is a stationary point if and only if it satisfies
% \begin{align}
%     \left(1 - \alpha \sigma'(2w)^2 - \alpha \sigma(2w) \sigma''(2w) + \alpha \sigma(w_{1,\ast}) \sigma''(2w)\right)( \sigma(2w - 2\alpha \sigma(2w)\sigma'(2w) + \alpha \sigma(2w_{1,\ast}) \sigma''(2w)  - \sigma(2w_{1,\ast})) \sigma'(2w - 2\alpha \sigma(2w)\sigma'(2w)+\alpha\sigma(2w_{1,\ast})\sigma'(2w))
% \end{align}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{NeurIPS/erm_log_eh.pdf}}
% \caption{
% }
% \label{maml_softplus_eh}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{NeurIPS/maml_log_eh.pdf}}
% \caption{
% }
% \label{maml_softplus_eh}
% \end{center}
% \vskip -0.2in
% \end{figure}


% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{NeurIPS/erm_log.pdf}}
% \caption{
% }
% \label{maml_softplus_eh}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.9\columnwidth]{NeurIPS/maml_log.pdf}}
% \caption{
% }
% \label{maml_softplus_eh}
% \end{center}
% \vskip -0.2in
% \end{figure}


 \begin{figure*}[t]
\begin{center}
%\centerline{\includegraphics[width=0.9\textwidth, height=3.9cm]{intro2.png}}
% for aistats 2 column, it was 0.21\textwidth
    %  \begin{subfigure}[b]{0.249\textwidth}
    \begin{subfigure}[b]{0.2488\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/erm_softplus_E_FINAL.pdf}
        \includegraphics[width=\textwidth]{NeurIPS/nal_loss_softplus_no_hard.pdf}
         \caption{}
         \label{fig:y equals x}
     \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.2435\textwidth}
     \begin{subfigure}[b]{0.2434\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/maml_softplus_E_FINAL.pdf}
        \includegraphics[width=\textwidth]{NeurIPS/maml_loss_softplus_no_hard.pdf}
         \caption{}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.249\textwidth}
    \begin{subfigure}[b]{0.2488\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/erm_softplus_EH_FINAL.pdf}
        \includegraphics[width=\textwidth]{NeurIPS/nal_loss_softplus_hard.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.237\textwidth}
     \begin{subfigure}[b]{0.2369\textwidth}
         \centering
        %  \includegraphics[width=\textwidth]{NeurIPS/maml_softplus_EH_FINAL.pdf}
        \includegraphics[width=\textwidth]{NeurIPS/maml_loss_softplus_hard.pdf}
         \caption{}
         \label{fig:five over x}
     \end{subfigure}
     \vspace{-1mm}
        \caption{
        Loss landscapes and ground-truth neurons for NAL (a,c) and MAML (b,d) for two distinct, four-task environments and Softplus activation.
        % Multi-task loss landscapes for one-layer neural networks with softplus activation (smoothed ReLU). excess risk of erm solution: 0.53. excess risk of maml solution: 0.34. , excess risk of erm solution: 0.19. excess risk of maml solution: 0.17.
        }
        % \label{fig:three graphs}
%\caption{Excess risks and optimal solutions for MAML and NAL in various types of task environments.}
% \vspace{-2mm}
\label{fig:softplus}
\end{center}
 \vskip -0.1in
\end{figure*}



==> NeurIPS/Problem_Formulation.tex <==
%!TEX root = main.tex
% \section{Problem setup: training to adapt} \label{section:pf}
\section{Problem Setup: Training to Adapt} \label{section:pf}

\vspace{-1mm}
% In many applications, models must quickly adapt to new tasks with limited accessible labeled data and computational resources.
% The MAML framework formalizes such scenarios by allowing the learner to update its model with one (or few) step(s) of stochastic gradient descent (SGD) at test time using a small number of samples from the task it will be evaluated on. 
% Our goal is to determine when and why the solution obtained by solving the MAML formulation leads to models that are more adaptable compared to models obtained by solving the traditional NAL problem. 
% we focus on a simple but fundamental example in which task is a linear regression.


% \textbf{Gradient-based meta-learning.} We are interested in the gradient-based meta-learning setting. Namely,
% In many applications, models must quickly adapt to new tasks with limited accessible labeled data and computational resources. 
We aim to determine when and why MAML yields models that are significantly more adaptable compared to models obtained by solving the traditional NAL problem in multi-task environments. To this end, we consider the gradient-based meta-learning setting in which a meta-learner tries to use samples from a set of tasks observed during meta-training to compute a model that performs well after one or a few steps of SGD on a new task drawn from the same environment at meta-test time.
%  This setting is general enough to capture numerous application areas, including few-shot learning \cite{} and federated learning \citep{fallah2020personalized}.
 
Specifically, we follow \cite{baxter1998theoretical} by considering an environment $p$ which is a distribution over tasks. Each task $\mathcal{T}_i$ is composed of a data distribution $\mu_i$ over an input space $\mathcal{X}$ and a label space $\mathcal{Y}$. We take our model class to be the family of functions $\{h_\mathbf{w} : \mathcal{X} \rightarrow \mathcal{Y}: \mathbf{w} \in \mathbb{R}^D\}$ where $h_{\mathbf{w}}$ is a model parameterized by $\mathbf{w}$. The population loss $f_i(\mathbf{w})$ on task $i$ is the expected value of  the loss of $h_\mathbf{w}$ on samples drawn from $\mu_i$, namely $f_i(\mathbf{w}) \coloneqq \mathbb{E}_{(\mathbf{x},y)\sim \mu_i}[\ell(h_\mathbf{w}(\mathbf{x}), y)]$, where $\ell$ is some loss function, such as the squared or cross entropy loss. 


% Ultimately we are interested in the ability of models to rapidly adapt to tasks drawn from the environment p. 

% define the risk of a model $\mathbf{w}$

% We will often need empirical estimates of the population losses, which we denote by $\hat{f}_i(\mathbf{w}; \mathbf{X},\mathbf{y}) \coloneqq $
 
% in general case, we need: 
% in general case, we need: 
 

% and updates the linear model $\mathbf{w}$ via one step of SGD using those $m$ samples. Finally, the updated model is evaluated by its regression error for unlabeled samples drawn from the same task.
%$n$ labeled samples from each of $T$ tasks drawn from some environment at training. The agent then computes an initial model $\mathbf{w}$ based on these $nT$ total data points. At test time, a {\em new} task is drawn from the environment along with $m$ labeled samples from that task. The agent adapts its initial model using a small number of gradient-based updates using the $m$ samples. MAML  to use the $nT$ training samples to find an initial model that performs optimally after these test-time updates, on average over tasks coming from the environment.

% We consider the realizable case in which each task is a regression problem involving the learning of a  single neuron. We let feature vectors $\mathbf{x}_i \in \mathbb{R}^d$ and their corresponding labels $y_i \in \mathbb{R}$ for the $i$-th task be jointly distributed according to $\mu_i$. Given an activation $\sigma: \mathbb{R} \rightarrow \mathbb{R}$, the population loss of the model $\mathbf{w} \in \mathbb{R}^d$ on the $i$-th task is the population mean squared error: $f_i(\mathbf{w}) \coloneqq \tfrac{1}{2}\mathbb{E}_{(\mathbf{x}_i,y_i) \sim \mu_i} [ ( \sigma(\mathbf{w}^\top \mathbf{x}_i) - y_i)^2 ]$. In the first part of the paper we will consider the special case when $\sigma$ is the identity map, but introduce the general case for now.

% The empirical loss of $\mathbf{w}$ on the $i$-th task given some data $\mathbf{}$


% Following \cite{baxter1998theoretical}, we assume tasks belong to an environment which is  a task
% distribution $p$. 
During training, the meta-learner samples $T$ tasks from $p$ and $n$ points $\{(\mathbf{x}_i^j, y_i^j)\}_{j=1}^n \sim \mu_i^n$ for each sampled task $\mathcal{T}_i$. 
% We denote $\mathbf{X}_i \in \mathbb{R}^{n \times d}$ and  $\mathbf{y}_i \in \mathbb{R}^n$ as the matrix and vector containing the training feature vectors and labels for the $i$-th task, respectively. 
The meta-learner uses this data to compute an initial model $\mathbf{w}$, which is then evaluated as follows. First, the meta-learner samples a new task $\mathcal{T}_i\sim p$ and $m$ labeled points $\{(\mathbf{\hat{x}}_i^j, \hat{y}_i^j) \}_{j=1}^m \sim \mu_i^m$. Next, it updates $\mathbf{w}$ with one step of stochastic gradient descent (SGD) on the loss function $f_i$ using those $m$ samples and step size $\alpha$. Namely, letting $\mathbf{\hat{X}}_i \in \mathbb{R}^{m \times d}$ and $\mathbf{\hat{y}}_i \in \mathbb{R}^{m}$ denote the matrix and vector containing the $m$ feature vectors and their labels, respectively, 
% where $\sigma(\cdot)$ is applied element-wise, 
the update of $\mathbf{w}$ is given by $\mathbf{w}_i \coloneqq \mathbf{w} - \alpha \nabla_{\mathbf{w}} \hat{f}_i(\mathbf{w}; \mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)$, where  $\hat{f}_i(\mathbf{w};\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)\!\coloneqq \! \frac{1}{m}\sum_{j=1}^m \ell(h_\mathbf{w}(\mathbf{\hat{x}}_i^j),\hat{y}_i^j)$ is the empirical average of the loss on the $m$ samples in $(\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)$.
%$\coloneqq \tfrac{1}{m} \sum_{j=1}^m \ell(\mathbf{w}; \mathbf{\hat{x}}_i^j, \hat{y}_i^j)$,
The test loss of $\mathbf{w}$ is the expected population loss of $\mathbf{w}_i$, where the expectation is taken over tasks and the $m$ samples, specifically
\begin{align} \label{exp_test}
    F_m(\mathbf{w}) &\coloneqq 
  \mathbb{E}_{i} \mathbb{E}_{(\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)} \big[ f_i(\mathbf{w}\! -\! \alpha \nabla \hat{f}_i(\mathbf{w};\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i ))\big]
\end{align}
% We assume the data for the $i$-th task is Gaussian and generated by a teacher neuron $\mathbf{w}_{i,
% \ast}$. In particular, points $(\mathbf{x}_i, y_i)$ are drawn from $\mu_i$ by first sampling $\mathbf{x}_i \sim \mathcal{N}(0,\mathbf{\Sigma}_i)$ then $y_i \sim \mathcal{N}(\sigma(\mathbf{w}_{i,\ast}^\top\mathbf{x}), \nu^2)$, i.e. $y_i = \mathbf{w}_{i,\ast}^\top\mathbf{x} + z_i$ where $z_i \sim \mathcal{N}(0,\nu^2)$.
% consider a task environment $p(\mathcal{T})$ which is a distribution over tasks $\mathcal{T}_i$. Each task $\mathcal{T}_i = (f_i,  \mathbf{w}_i^\ast, \mathbf{\Sigma}_i)$ consists of a loss function $f_i: \mathbb{R}^d \rightarrow \mathbb{R}$, an optimal solution $\mathbf{w}_i^\ast \in \mathcal{H}_i$, and a data covariance matrix $\mathbf{\Sigma}_i \in \mathbb{R}^{d \times d}$. We will let ${\mathcal{H}_i} = \mathbb{R}^d$ for all $i$. 
% With slight abuse of terminology, we sometimes use ``locations of tasks'' to refer to the locations of the tasks' optimal solutions.
% Samples $(\mathbf{x}_i,y_i)$ from the $i$-th task are drawn by first sampling $\mathbf{x}_i \sim \mathcal{N}(\mathbf{0}_d,\mathbf{\Sigma}_i)$ then %$y_i \sim \mathcal{N}(\mathbf{x}_i^\top \mathbf{w}_i^\ast,\sigma_i^2 )$, or equivalently,
% computing $y_i = \mathbf{x}_i^\top \mathbf{w}_i^\ast + z_i$ where $z_i \sim \mathcal{N}({0}, \sigma^2)$. The loss function $f_i(\mathbf{w})$ for the $i$-th task is the mean squared error over samples drawn from the $i$-th task, namely $f_i(\mathbf{w}) = \frac{1}{2}\mathbb{E}_{ (\mathbf{x}_i,y_i)}  \left[(\langle \mathbf{w}, \mathbf{x}_i \rangle - y_i)^2\right]$. Denoting the $m$ samples from task $i$ used to update the model at test time with the matrix $\mathbf{\hat{X}}_i \in \mathbb{R}^{m \times d}$, whose rows are the feature vectors, and the vector $\mathbf{\hat{y}}_i \in \mathbb{R}^{m}$, whose elements are the corresponding labels, then the empirical loss of $\mathbf{w}$ on these samples is 
% $\hat{f}_i(\mathbf{w}, (\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)) = \frac{1}{2n} \| \mathbf{\hat{X}}_i \mathbf{w} - \mathbf{\hat{y}}_i \|_2^2$. 
% %We denote the training samples for the $i$-th task as $\{(\mathbf{x}_i^{(j)}, y_i^{(j)})\}_{j=1}^n$ and the samples available to the learner at test time using the matrix $\mathbf{\hat{X}}_i \in \mathbb{R}^{m \times d}$, whose rows are the $m$ feature vectors, and the vector $\mathbf{\hat{y}}_i \in \mathbb{R}^{m}$ containing their corresponding labels. 
% The test error of the model $\mathbf{w}$ is then:
% \begin{align} \label{exp_test}
%     F_m(\mathbf{w}) &\coloneqq 
%   \mathbb{E}_{i, (\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)} \big[ f_i(\mathbf{w}\! -\! \alpha \nabla \hat{f}_i(\mathbf{w},(\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i) ))\big]
% \end{align}
% where we used the shorthand notation $ \mathbb{E}_{i}$ to denote $\mathbb{E}_{i \sim p(\mathcal{T})}$, as we use throughout the paper, and 
% %each $F_i(w) = \mathbb{E}_{(\hat{X}_i, \hat{y}_i)} f_i(w - \alpha \nabla_w \hat{f}_i(w, (\hat{X}_i, \hat{y}_i)))$ is the meta-loss for the $i$-th task, and 
% $\alpha$ is the step size. 
where we have used the shorthand $\mathbb{E}_{i}\!\coloneqq\! \mathbb{E}_{\mathcal{T}_i\sim p}$ and $\mathbb{E}_{(\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i)} \!\coloneqq\! \mathbb{E}_{(\mathbf{\hat{X}}_i, \mathbf{\hat{y}}_i) \sim \mu_i^m}$.
For fair evaluation, we 
% ignore loss terms containing uncontrollable noise and
measure solution quality by the excess risk
\begin{align} \label{eq:excess_risk}
    \mathcal{E}_m(\mathbf{w}) &\coloneqq F_m(\mathbf{w}) -  \inf_{\mathbf{w}' \in \mathbb{R}^D} F_m(\mathbf{w}')
    % \tfrac{1}{2} \mathbb{E}_{i}\big[ \sigma^2 + \tfrac{\alpha^2 \sigma^2}{m} \text{tr} ( \mathbf{\Sigma}_i^2)\big] = \tfrac{1}{2}  \mathbb{E}_{i,\mathbf{\hat{X}}_i}\big \| \mathbf{\tilde{P}}_i(\mathbf{w} - \mathbf{w}_i^\ast) \|^2_{\mathbf{\Sigma}_i}\big],
\end{align}
% where $\mathbf{\hat{P}}_i \coloneqq \mathbf{I}_d -  \tfrac{\alpha}{m}\mathbf{\hat{X}}_i^\top \mathbf{\hat{X}}_i$ for all $i$. 
% The excess risk is the difference 
The excess risk is the difference between the average performance of $\mathbf{w}$ after one step of task-specific adaptation from the performance of the best possible initialization for fast adaptation. %, which is ultimately the metric we are interested in minimizing.
% Our ultimate goal is to find a model that performs as well as the best possible model after one step of task-specific adaptation on average, which is equivalent to seeking a model $\mathbf{w}$ that has a small excess risk. 
% To achieve this goal, we can solve one of two problems during training, NAL or MAML.
To find a model with small excess risk, one can solve one of two problems during training, NAL or MAML.

\vspace{0.6mm}
\noindent \textbf{NAL.} NAL minimizes the loss $f_i(\mathbf{w})$ on average across the training tasks, which may yield small excess risk $\mathcal{E}_m(\mathbf{w})$ with less computational cost than MAML \citep{gao2020modeling}. 
% Indeed, the occasional strength of NAL for learning an initialization for SGD have been pointed out in \cite{gao2020modeling}. 
Denoting the $n$ training examples for the $i$-th task as $\mathbf{{X}}_i \!\in\! \mathbb{R}^{n \times d}$ and their labels as $\mathbf{{y}}_i \!\in\! \mathbb{R}^{n}$, 
%$\{(\mathbf{x}_i^{(j)}, y_i^{(j)})\}_{j=1}^n$ at training time for each task $i$, the empirical loss of $\mathbf{w}$ on these samples is defined as 
% $\hat{f}_i(\mathbf{w}, \{(\mathbf{x}_i^{(j)}, y_i^{(j)})\}_{j=1}^n)\ :=\ \frac{1}{2n}\sum_{j=1}^n (\langle \mathbf{w}, \mathbf{x}_i^{(j)}\rangle  - y_i^{(j)} )^2.
% $ In matrix form, with the $n$ feature vectors contained in the rows of the matrix $\mathbf{\bar{X}}_i$ and the labels contained in $\mathbf{\bar{y}}_i$, this loss can be rewritten as $\hat{f}_i(\mathbf{w}, (\mathbf{\bar{X}}_i, \mathbf{\bar{y}}_i)) = \frac{1}{2n} \| \mathbf{\bar{X}}_i \mathbf{w} - \mathbf{\bar{y}}_i \|_2^2$. 
NAL %finds the model that achieves the smallest average loss on the $T$ train tasks, i.e. it 
solves
\begin{align} \label{emp_orig}
    \min_{\mathbf{w}\in \mathbb{R}^D} {F}^{tr}_{NAL}(\mathbf{w}) &\coloneqq \tfrac{1}{T} \textstyle\sum_{i=1}^T \hat{f}_i(\mathbf{w}; \mathbf{X}_i, \mathbf{y}_i),  
    %\| \mathbf{\bar{X}}_i \mathbf{w} - \mathbf{\bar{y}}_i \|_2^2.
\end{align}
which is a surrogate for the expected risk minimization problem defined as
% $
%     \min_{\mathbf{w}\in \mathbb{R}^d}\ 
%  \mathbb{E}_{i} \left[f_i(\mathbf{w})\right] = \tfrac{1}{2} \mathbb{E}_{i} \left[ \mathbb{E}_{\mathbf{x}_i,y_i} \left[ ( \langle \mathbf{w},  \mathbf{x}_i \rangle -y_i)^2\right]\right]
% $.
$
    \min_{\mathbf{w}\in \mathbb{R}^D}\ 
 \mathbb{E}_{i} \left[f_i(\mathbf{w})\right]
 %= \mathbb{E}_{i} \left[ \mathbb{E}_{\mathbf{x}_i,y_i} \left[ ( \langle \mathbf{w},  \mathbf{x}_i \rangle -y_i)^2\right]\right]
$.
%\textcolor{red}{It can easily be shown that the objective function in \eqref{emp_orig} is strongly convex}, so 
We let $\mathbf{w}_{NAL}^\ast$ denote the unique solution of the expected risk minimization problem, and let $\mathbf{w}_{NAL}$ denote the unique solution to (\ref{emp_orig}). We emphasize that in our study we evaluate the solution of NAL by its expected error after running one step of SGD using the $m$ samples from a new task that are released at test time, and this error is captured by the excess risk $\mathcal{E}_m(\mathbf{w}_{NAL})$, defined in (\ref{eq:excess_risk}).

\vspace{0.6mm}
\noindent \textbf{MAML.} In contrast to NAL, MAML  minimizes a surrogate loss of (\ref{exp_test}) during training. 
% To account for the expectation over the stochastic gradient that is outside of the function evaluation in (\ref{exp_test}), 
According to the MAML framework, the $n$ samples per task are divided into $\tau$ training ``episodes'', each with  $n_2$ ``inner" samples for the inner SGD step and $n_1$ ``outer" samples for evaluating the loss of the fine-tuned model. Thus, we have that
% the total number of training samples available for each task is 
$\tau(n_1+n_2) = n$. We denote the matrices that contain the outer samples for the $j$-th episode of the $i$-th task as $\mathbf{X}_{i,j}^{out} \in \mathbb{R}^{n_1 \times d}$ and $\mathbf{y}_{i,j}^{out} \in \mathbb{R}^{n_1}$, and the matrices that contain the inner samples as $\mathbf{{X}}_{i,j}^{in} \in \mathbb{R}^{n_2 \times d}$ and $\mathbf{{y}}_{i,j}^{in} \in \mathbb{R}^{n_2}$. The MAML objective is then
\begin{equation}\label{emp_maml}
    \min_{\mathbf{w}\in \mathbb{R}^D}\ 
   {F}_{MAML}^{tr}(\mathbf{w}) \coloneqq 
%   \frac{1}{T\tau }\sum_{i=1}^T \sum_{j=1}^\tau  \|\mathbf{X}_{i,j}(\mathbf{w}\! -\! \tfrac{\alpha}{n_2}\mathbf{\hat{X}}_{i,j}^\top   (\mathbf{\hat{X}}_{i,j} \mathbf{w}\! -\! \mathbf{\hat{y}}_{i,j}))  \!-\! \mathbf{y}_{i,j}\|^2_2
   \tfrac{1}{T\tau } \sum_{i=1}^T \sum_{j=1}^\tau \hat{f}_i(\mathbf{w} - \alpha \nabla \hat{f}_i(\mathbf{w};\mathbf{{X}}^{in}_{i,j}, \mathbf{{y}}^{in}_{i,j} ); \mathbf{{X}}^{out}_{i,j}, \mathbf{{y}}^{out}_{i,j}).
\end{equation}
%Assume that we have $n_1$ samples for evaluating the outer loop meta-training error, thus $X_1, X_2 \in \mathbb{R}^{n_1 \times 2}$ and $y_1, y_2 \in \mathbb{R}^{n_1}$. Meanwhile, we have $n_2$ samples for performing the inner gradient step, thus $\hat{X}_1, \hat{X}_2 \in \mathbb{R}^{n_2 \times 2}$ and $\hat{y}_1, \hat{y}_2 \in \mathbb{R}^{n_2}$. All samples are drawn independently. 
We denote the unique solution to (\ref{emp_maml}) by $\mathbf{w}_{MAML}$ and the unique solution to the population version (\ref{exp_test}) by $\mathbf{w}_{MAML}^\ast$. We expect $\mathcal{E}_m(\mathbf{w}_{MAML}) \leq \mathcal{E}_m(\mathbf{w}_{NAL})$ since (\ref{emp_maml}) is a surrogate for the true objective of minimizing (\ref{exp_test}). However, the gain of MAML over NAL may not be significant enough to justify its added computational cost \citep{gao2020modeling}, necessitating a thorough understanding of the relative behavior of MAML and NAL.


% $\mathbf{w}_{MAML}$ converges slowly to $\mathbf{w}_{MAML}^\ast$, the minimizer of (\ref{exp_test}), while $\mathcal{E}_m(\mathbf{w}_{NAL})$ is relatively small, in which case $\mathcal{E}_m(\mathbf{w}_{MAML}) \approx \mathcal{E}_m(\mathbf{w}_{NAL})$. 
% In the subsequent sections we  illustrate the conditions under which $\mathcal{E}_m(\mathbf{w}_{MAML}) \ll \mathcal{E}_m(\mathbf{w}_{NAL})$.

% and compare its performance to that of $\mathbf{w}_{NAL}$ on the excess risk $\mathcal{E}_m$ in the following sections.



==> Related_Work.tex <==
%!TEX root = main.tex


%\section{RELATED WORK} 
%The MAML framework \citep{finn2017model}
%draws from the meta-learning setup initially proposed in \cite{baxter1998theoretical}. 
% \noindent \textbf{Related Work.} 
\subsection{Related work} 
% \textbf{Model-Agnostic Meta-Learning.} 
% MAML and its closely-related variants have been the focus of many empirical studies in recent years \citep{antoniou2018train,nichol2018reptile,li2017meta,zintgraf2019fast}. 
% Despite thorough empirical analyses
% motivated by evidence of MAML's strong empirical few-shot learning performance \cite{finn2017model,antoniou2018train}
% Theoretical analysis of MAML has included showing 

A few works have explored why MAML is effective. 
% \cite{goldblum2020unraveling} demonstrated empirically that some meta-learning algorithms learn more clustered features compared to standard training, although this does not apply to MAML. \citet{jose2021information} showed that task environments with similar tasks allow for meta-learners that generalize well. 
\cite{raghu2019rapid} posed two hypotheses for MAML's success in training neural networks: {\em rapid learning}, meaning that MAML finds a set of parameters advantageous for full adaptation on new tasks, and {\em feature reuse}, meaning that MAML learns a set of reusable features, among the tasks. The authors' experiments showed that MAML learns a shared representation, supporting the feature reuse hypothesis. Motivated by this idea, \cite{saunshi2020sample} proved that Reptile \citep{nichol2018reptile}, a similar algorithm to MAML, can learn a representation that reduces the new-task sample complexity in a two-task, linear setting. 
% \cite{chua2021fine} argued that adapting the representation during meta-test time is necessary to achieve the dimensionality-reduction benefits of representation-learning in a linear setting in which the ground-truth representation for each task is a perturbed version of the shared representation, but they did not show any benefit of adapting the representation during meta-training. 
Conversely, \cite{oh2020does} gave empirical evidence that MAML performance does not degrade when forced to learn unique representations for each task, 
% and  \cite{goerttler2021exploring} gave empirical evidence suggesting that shared repr
and \cite{goldblum2020unraveling} showed that while some meta-learning algorithms learn more clustered features compared to standard training, the same cannot be said of MAML. % due to its inner loop update of the representation parameters.
Moreover, a series of works have shown that removing the inner loop and learning a distinct classifier for each class of images in the environment can yield representations as well-suited for few-shot image classification as MAML's \citep{chen2019closer}. In this work, we take a more general, landscape-based perspective on the reasons for MAML's success, and show that MAML can still achieve meaningful gain without necessarily learning a representation.


%that nearly all of MAML's performance is sustained when the body of the neural network is fixed during inner loop updates, suggesting that MAML reuses features on new tasks. 
%empirical evidence to support the former. In particular, they showed that a variant of MAML that does not update the body of the neural network used as a learning model during the inner loop, termed ANIL, performs nearly as well as MAML for few-shot classification tasks, suggesting that MAML reuses the feature representations learned previous tasks without updating them for a new task. 


%showed that fixing the network head during the inner loop also does not significantly affect performance, 
% empirically argued that MAML enables fast adaptation because it learns a rapidly adaptable feature representation. %, which is supported by recent theoretical work \citep{}. 
%a variant of MAML in which \textit{only} the body, and not the head, is updated during the inner loop, namely BOIL, also performs nearly as well as MAML, suggesting that MAML learns a feature representation that is suitable to rapid updates on new tasks.
%Meanwhile, \cite{goldblum2020unraveling} demonstrated empirically that some meta-learning algorithms learn more clustered features compared to standard training, although their argument does not apply to MAML. 
%Similarly, \cite{khodak2019provable} observed that the 
%because it does not fix the feature extractor (network body) during the inner loop.
% A number of works have attempted to theoretically explain meta-learning's effectiveness by
% considering a very similar mixed linear regression setting as ours.
% \cite{goldblum2020unraveling} showed  that a set of meta-learners which fix the representation during the inner loop (MetaOptNet and R2D2) learn representations that cluster the features from different image classes. However, they also show that MAML, which does not fix the feature extractor during the inner loop, does not exhibit this property.
% Meanwhile, other studies of MAML and related methods have 
%  explored the 

% \textbf{Linear meta-learning.} 

Much of the theory surrounding MAML and meta-learning more broadly has focused on linear settings, specifically multi-task linear regression or the related linear centroid problem \citep{denevi2018learning}. Some works have studied how to allocate data amongst and within tasks  \citep{cioba2021distribute, bai2020important, saunshi2021representation}. \citet{denevi2018learning} considered meta-learning a common mean for ridge regression, and \cite{kong2020meta} studied whether many small-data tasks and few large-data tasks is sufficient for meta-learning.
Other works have examined the role of the inner loop SGD step size in meta-learning approaches \citep{bernacchia2021meta,charles2020outsized,wang2020guarantees}, while
% for general quadratic objectives,
% but focused on convergence rates rather than the test performance of particular solutions 
\cite{gao2020modeling} studied the trade-off between the accuracy and computational cost of the NAL and MAML training solutions. However, unlike our work, these works either did not consider or did not provide any interpretable characterization of the types of task environments in which MAML is effective.
% \cite{du2020few} and \cite{tripuraneni2020provable} showed that if there exists a subspace containing the tasks' optimal solutions, then it can be learned in a sample-efficient manner via NAL, while
% while \cite{collins2021exploiting, thekumparampil2021sample} provided efficient algorithms for learning 
% \cite{chua2021fine} proved that if each task has a perturbed representation, then fine-tuning the representation on a new task is necessary to realize the dimensionality-reduction benefits of representation learning.
% Moreover, \cite{saunshi2020sample} demonstrated that learning the subspace is necessary to reduce the dimension-dependence in the new-task sample complexity in a specific two-task environment. 
% Our work is orthogonal in that it shows that specifically MAML, not a generic meta-learning framework, can achieve meaningful gain in excess risk without assuming the tasks' solutions exactly or approximately belong to a shared subspace.
% , in terms of excess risk for a fixed sample size and computational budget.
%Meanwhile, Ge et al analyzed the ... also sewoong paper
% some have focused on the role of data-splitting \citep{bai2020important, saunshi2021representation}
 %limiting the practicality of their discussion.
% \cite{kao2021maml} 
% studied whether many small-data tasks and few large-data tasks is sufficient for meta-learning, 
% \cite{bernacchia2021meta} analyzed the choice of inner loop step size for MAML in the multi-task linear regression setting
Other theoretical studies of MAML and related methods have focused on convergence rates in general settings
\citep{fallah2020convergence, rajeswaran2019meta, zhou2019efficient, ji2020convergence, ji2020theoretical, collins2020task, wang2020global} and excess risk bounds for online learning \citep{finn2019online, balcan2019provable, khodak2019adaptive}. Like the current work, \cite{fallah2020convergence} noticed that the MAML solution should be closer than the NAL solution to the hard tasks' global minima, but the authors neither quantified this observation nor further compared MAML and NAL.  
\vspace{-2mm}
% the optimal meta-generalization gap of a meta-learner is inversely related to similarity of the tasks in the task environment

% More papers to cite:
% - sun and zhou hardness papers.
% - support set diversity paper
% - bo liu optimization paper?
% - no inner loop iclr paper
% - train test val split
% - 

%\cite{wang2020guarantees} provided guarantees for meta-learning the SGD step size for quad

%Also, \cite{zhou2020expert} analyzed task hardness in meta-learning
%Different types of hardness in classification: semantic, confusion, distance (mention these in experiment section)

%.\footnote{As others have noticed \cite{charles2020outsized}, the preconditioned covariance matrix $\mathbf{\Sigma}_i \left( \mathbf{I}_d- \alpha \mathbf{\Sigma}_i \right)^2$ has smaller condition number than the original covariance matrix $\mathbf{\Sigma}_i$. %, so for sufficiently large $a$, we have $\tfrac{L_a}{\mu_a} \leq \tfrac{L}{\mu}$.}

% \noindent \textbf{Effectiveness of Meta-Learning.}
%\noindent \textbf{Mixtures of Linear Regression.}

% ways to improve paper:
% 1. modify theorems 3 and 4 to account for easy and hard tasks, then comment on performance tradeoff... ithink this would be too complicated
% 2. modify theorem 4 to account for n2 vs tau tradeoff.. but this is an orthogonal point
% 3. figures for effect of task hardness on sigmoid landscape, closeness of maml to the solution predicted by upper bounds.
% 4. figures for the effect of task geography on sigmoid landscape - two with large RH, small RE, then two with the opposite
% 5. problem formulation needs to be for general function classes first
% sections: RW, PF-general, Mixed Linear (preliminaries - maml and erm population and empirical solutions and prop 1, task hardness, task geography and corollary 1), nonlinear (preliminaries, task hardness, task geo), experiments (task hardness and task geo)

